Multi-Pass Graph Streaming Lower Bounds for Cycle Counting, MAX-CUT, Matching Size, and Other Problems

Consider the following gap cycle counting problem in the streaming model: The edges of a $2$-regular $n$-vertex graph $G$ are arriving one-by-one in a stream and we are promised that $G$ is a disjoint union of either $k$-cycles or $2k$-cycles for some small $k$; the goal is to distinguish between these two cases. Verbin and Yu [SODA 2011] introduced this problem and showed that any single-pass streaming algorithm solving it requires $n^{1-\Omega(\frac{1}{k})}$ space. This result and the technique behind it -- the Boolean Hidden Hypermatching communication problem -- has since been used extensively for proving streaming lower bounds for various problems. Despite its significance and broad range of applications, the lower bound technique of Verbin and Yu comes with a key weakness that is inherited by all subsequent results: the Boolean Hidden Hypermatching problem is hard only if there is exactly one round of communication and can be solved with logarithmic communication in two rounds. Therefore, all streaming lower bounds derived from this problem only hold for single-pass algorithms. We prove the first multi-pass lower bound for the gap cycle counting problem: Any $p$-pass streaming algorithm that can distinguish between disjoint union of $k$-cycles vs $2k$-cycles -- or even $k$-cycles vs one Hamiltonian cycle -- requires $n^{1-\frac{1}{k^{\Omega(1/p)}}}$ space. As a corollary of this result, we can extend many of previous lower bounds to multi-pass algorithms. For instance, we can now prove that any streaming algorithm that $(1+\epsilon)$-approximates the value of MAX-CUT, maximum matching size, or rank of an $n$-by-$n$ matrix, requires either $n^{\Omega(1)}$ space or $\Omega(\log{(\frac{1}{\epsilon})})$ passes. For all these problems, prior work left open the possibility of even an $O(\log{n})$ space algorithm in only two passes.

==> Files/fig-re.tex <==
% !TeX root = ../main.tex 
%!TEX root = ../main.tex

\begin{tikzpicture}
%	\node[ellipse, black, fill=black!10, draw, line width=1pt, minimum width=40pt, minimum height=100pt] (V1) {};
\tikzset{vertex/.style={circle, black, fill=Yellow, line width=1pt, draw, inner sep=0pt, minimum width=8pt, minimum height=10pt}}
\tikzset{vset/.style={rectangle, rounded corners, black, fill=black!0, draw, line width=1pt, inner sep=0pt, minimum width=18pt, minimum height=90pt}}

\node[vset] (A0){};
\node [vertex] (A0y0) at ($(A0)+(0,36pt)$) {};
	\foreach \y in {1,...,4} 
       	 {
      		\pgfmathtruncatemacro{\yy}{\y-1}
		\node [vertex] (A0y\y) at ($(A0y\yy)+(0,-18pt)$) {};
	}
		
\foreach \x in {1,...,10}{
 	 \pgfmathtruncatemacro{\xx}{\x-1}

	\node[vset](A\x)[right=25pt of A\xx]{};
		\node [vertex] (A\x y0) at ($(A\x)+(0,36pt)$){};
		 \foreach \y in {1,...,4} 
       		 {
      			\pgfmathtruncatemacro{\yy}{\y-1}
			\node [vertex] (A\x y\y) at ($(A\x y\yy)+(0,-18pt)$){};
		}
}

\foreach \x in {0,...,5}{
 	\pgfmathtruncatemacro{\xx}{2*\x}
	\node[vset](B\x)[below=30pt of A\xx]{};
		\node [vertex] (B\x y0) at ($(B\x)+(0,36pt)$){};
		\foreach \y in {1,...,4} 
       	{
      		\pgfmathtruncatemacro{\yy}{\y-1}
			\node [vertex] (B\x y\y) at ($(B\x y\yy)+(0,-18pt)$){};
		}
}

% \foreach \x in {0,2,4}{
% 	\pgfmathtruncatemacro{\xx}{2*\x}
%  	\pgfmathtruncatemacro{\xxx}{2*\x+2}

%  	\draw [rectangle, dashed, rounded corners, gray, line width=1.5pt] ($(A\xx)+(-12pt, -48pt)$) rectangle ($(A\xxx)+(12pt,52pt)$);
% }
% \foreach \x in {1,3}{
% 	\pgfmathtruncatemacro{\xx}{2*\x}
%  	\pgfmathtruncatemacro{\xxx}{2*\x+2}

%  	\draw [rectangle, dashed, rounded corners, gray, line width=1.5pt] ($(A\xx)+(-12pt, -52pt)$) rectangle ($(A\xxx)+(12pt,48pt)$);
% }

\foreach \x in {0,2,4,6,8}{
	\foreach \y in {0,...,4}{
		\pgfmathtruncatemacro{\xx}{\x+1}
		\pgfmathtruncatemacro{\yy}{Mod(\y+\x,5)}
		 
	 	\draw[line width=1pt, blue]
			(A\x y\y.east) -- (A\xx y\yy.west);
	}
}
\foreach \x in {0,1,2,3,4} {
	\pgfmathtruncatemacro{\xx}{2*\x}
	\node [above right=3pt and -2pt of A\xx]{\textcolor{blue}{$\Mb{\x}_1$}};
}

\foreach \x in {1,3,5,7,9}{
	 \foreach \y in {0,...,4}{
	 	 \pgfmathtruncatemacro{\xx}{\x+1}
		 \pgfmathtruncatemacro{\yy}{Mod(2*\y+\x,5)}
		 
	 	\draw[line width=1pt, red]
			(A\x y\y.east) -- (A\xx y\yy.west);
	 }
}

\foreach \x in {1,2,3,4}{
	\pgfmathtruncatemacro{\xx}{2*\x-1}
	\node [above right=3pt and -2pt of A\xx]{\textcolor{red}{$\Mb{\x}_2$}};	
}

% \node (m0) [above right=0pt and 41pt of B0]{\textcolor{blue}{Bob$_\theta$}};
\foreach \x in {0,2,4}{
	\pgfmathtruncatemacro{\xx}{\x+1}
	\foreach \y in {0,...,4}{
	\pgfmathtruncatemacro{\yy}{Mod(2*\y+\x+1,5)}	
	\draw[line width=1pt, orange]
		(B\x y\y.east) -- (B\xx y\yy.west);
	}
}
\foreach \x in {1,3}{
	\pgfmathtruncatemacro{\xx}{\x+1}
	\foreach \y in {0,...,4}{
	\pgfmathtruncatemacro{\yy}{Mod(2*\y+\x+1,5)}
	\draw[line width=1pt, gray]
		(B\x y\y.east) -- (B\xx y\yy.west);
	}
}
\node [above right=0pt and 25pt of B0]{\textcolor{orange}{$P_1$}};
\node [above right=0pt and 25pt of B1]{\textcolor{gray}{$P_2$}};
\node [above right=0pt and 25pt of B2]{\textcolor{orange}{$P_3$}};
\node [above right=0pt and 25pt of B3]{\textcolor{gray}{$P_4$}};


\end{tikzpicture}



==> Files/round-elimination.tex <==
% !TeX root = ../main.tex 
%!TEX root = ../main.tex


\def\new{\mathsf{new}}
\def\disty{\mathcal{U}'}
\def\Z{\mathsf{Z}}
\def\init{\mathsf{Init}}
\def\ext{\mathsf{Ext}}
\def\ev{\text{even}}
\def\od{\text{odd}}

\newcommand{\TODO}[1]{ {\color{red} #1 }}

\section{The Round-Elimination Argument (\Cref{lem:round-elimination})}\label{sec:round-elimination}



We prove~\Cref{lem:round-elimination}, restated below, in this section. Recall that $\adv(\cdot)$ is defined in \Cref{def:adv}.

\begin{restate}[\Cref{lem:round-elimination}]
	\lemroundeliminationcont
\end{restate}
\begin{proof}

For the rest of this section, we fix $\hat{\Y}$ and $\hat{\N}$ to be the maximizer of the left hand side and define $\Delta = \hat{Y}^{-1} \circ \hat{\N}$. We use $r \geq 2$ to denote the number of elements in $S$, and define $\disty$ to be the uniform distribution over all bijections $\Y: V_{S',c,0} \to V_{S',c,\n_{S',c}}$. In order to show the lemma, we actually show that:

\begin{lemma}
\label{lemma:reactual}
Let $\prot$ be an $r$-round $C$-length protocol for the $(S,c,\hat{\Y},\hat{\N})$-\FMT problem. For all bijections $\Y \in \supp{\disty}$, there is an $(r-1)$-round $C$-length protocol $\psi_{\prot, \Y}$ for the $(S',c,\Y,\Y \circ \Delta)$-\FMT problem such that:
\begin{align}
\tvd{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\Y}}_{S, c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y}_{S',c} } } &\leq  \frac{1}{2} \cdot \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .    \label{eq:reactualyes} \\
\tvd{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\N}}_{S, c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y \circ \Delta}_{S',c} } } &\leq  \frac{1}{2} \cdot \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .    \label{eq:reactualno} 
\end{align}
\end{lemma}
We defer the proof of \Cref{lemma:reactual} to later but use it now to finish the proof of \Cref{lem:round-elimination}. Using the notation of \Cref{lemma:reactual}, we have for all protocols $\prot$ that
\begin{align*}
&\tvd{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\Y}}_{S, c} } }{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\N}}_{S, c} } } \\
&\hspace{1cm}\leq \tvd{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\Y}}_{S, c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y}_{S',c} } } \\
&\hspace{3cm} + \tvd{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y}_{S',c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y \circ \Delta}_{S',c} } } \\
&\hspace{5cm} + \tvd{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y \circ \Delta}_{S',c} } }{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\N}}_{S, c} } } \tag{Triangle inequality} \\
&\hspace{1cm}\leq  \tvd{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y}_{S',c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist^{\Y \circ \Delta}_{S',c} } }  \\
&\hspace{7cm} +\sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} \tag{\Cref{lemma:reactual}} \\
&\hspace{1cm}\leq  \tvd{ \E_{\Y \sim \disty}\Bracket{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ G' \sim \dist^{\Y}_{S',c} } } }{ \E_{\Y \sim \disty}\Bracket{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ G' \sim \dist^{\Y \circ \Delta}_{S',c} } } }  \\
&\hspace{7cm} +\sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} \\
&\hspace{1cm}\leq  \E_{\Y \sim \disty}\Bracket{ \tvd{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ G' \sim \dist^{\Y}_{S',c} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ G' \sim \dist^{\Y \circ \Delta}_{S',c} } } }  + \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} \tag{\Cref{lemma:tvdtriangle}} \\
&\hspace{1cm}\leq  \E_{\Y \sim \disty}\Bracket{ \adv(C,S',c,\Y,\Y \circ \Delta) }  + \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} \tag{\Cref{def:adv}} \\
&\hspace{1cm}\leq \max_{ \substack{\Y, \N : V_{S',c,0} \to V_{S',c,\n_{S',c}} \\ \Y \neq\N \text{ are bijections}} } \adv(C,S',c,\Y,\N) +  \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .
\end{align*}
Taking the supremum over all protocols $\prot$ on the left hand side and applying \Cref{def:adv} finishes the proof of \Cref{lem:round-elimination}.
\end{proof}

It remains to show \Cref{lemma:reactual}, and we do that now. 
\begin{proof}[Proof of \Cref{lemma:reactual}]
Fix an $r$-round $C$-length protocol $\prot$ and observe that we can assume without loss of generality that $\prot$ is deterministic. Indeed, if we show \Cref{lemma:reactual} for all deterministic protocols, then from \Cref{lemma:tvdtriangle} and the fact that a randomized protocol is simply a distribution over deterministic protocols, we also get \Cref{lemma:reactual} for randomized protocols. For a bijections $\Y: V_{S',c,0} \to V_{S',c,\n_{S',c}}$, we define the protocol $\psi_{\prot, \Y}$ in \Cref{algo:psi}. 

Recall from \Cref{prob:FMT} that the input to $\psi_{\prot, \Y}$ is an $(S',c)$-nested block graph $G'$. While describing and analyzing \Cref{algo:psi}, we use primes to denote objects associated with $S'$ and $G'$ and letters without primes to denote objects associated with $S'$ and $G'$. For example, $V'$ will denote $V_{S', c}$, $\n'$ will denote $\n_{S', c}$, $\dist^{\hat{\N}}$ denotes the distribution $\dist^{\hat{\N}}_{S,c}$, {\em etc.} 

\begin{algorithm}[H]
\caption{The protocol $\psi_{\prot, \Y}$.}
\label{algo:psi}
\begin{algorithmic}[1]

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\Require As $(S',c)$-nested block graph $G' = \left( \bigsqcup_{i=0}^{\n'} V'_{i}, \bigsqcup_{i=1}^{\n'} E'_{i} \right)$. Alice is given the set of edges $\{E'_{i}\}_{\ev~i \in [\n']}$ and Bob is given the set of edges $\{E'_{i}\}_{\od~i \in [\n']}$. Both the players know the partition $V' = \bigsqcup_{i=0}^{\n'} V'_{i}$.

\bigskip

\Statex \hspace{-\algorithmicindent} {\bf Sample an $(S,c)$-nested block graph $G = \left( \bigsqcup_{i=0}^{\n} V_{i}, \bigsqcup_{i=1}^{\n} E_{i} \right)$ and a message $\Pi_1$:}

\bigskip

\State Using public randomness, sample $\{E_{i}\}_{i = \n - c + 1}^{\n}$ uniformly conditioned on $G^{\star}_{\n - c \to \n} = \hat{\Y} \circ \Y^{-1}$. \label{line:psi:last}

\bigskip

\State Using public randomness, sample $E_{(i-1)c + j}$ uniformly at random for all $i \in [\n']$ and $j \in [c]$ such that $i - j$ is even. \label{line:psi:even}

\bigskip

\State Alice, using her private randomness, samples edges $E_{(i-1)c + j}$ for all even $i \in [\n']$ and odd $j \in [c]$ uniformly conditioned on:
\begin{compactitem}
\item $\rv{E}_{(i-1)c + j} = E_{(i-1)c + j}$ for all even $i \in [\n']$ and even $j \in [c]$,
\item $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all even $i \in [\n']$.
\end{compactitem} \label{line:psi:alice1}

\bigskip 

\State Alice, using her private randomness, samples a message $\Pi_1$ from $\distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} }$ conditioned on:
\begin{compactitem}
\item $\{\rv{E}_{i}\}_{i = \n - c + 1, \ev~i}^{\n} = \{E_{i}\}_{i = \n - c + 1, \ev~i}^{\n}$,
\item $\rv{E}_{(i-1)c + j} = E_{(i-1)c + j}$ for all $i \in [\n']$ and $j \in [c]$ such that $i - j$ is even,
\item $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all even $i \in [\n']$.
\end{compactitem} \label{line:psi:alice2}

\bigskip

\State Alice sends $\Pi_1$ to Bob. \label{line:psi:comm1}

\bigskip

\State Bob, using his private randomness, samples edges $E_{(i-1)c + j}$ for all odd $i \in [\n']$ and even $j \in [c]$ uniformly conditioned on:
\begin{compactitem}
\item $\rv{\Pi}_1 = \Pi_1$, 
\item $\{\rv{E}_{i}\}_{i = \n - c + 1, \ev~i}^{\n} = \{E_{i}\}_{i = \n - c + 1, \ev~i}^{\n}$,
\item $\rv{E}_{(i-1)c + j} = E_{(i-1)c + j}$ for all $i \in [\n']$ and $j \in [c]$ such that $i - j$ is even,
\item $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all odd $i \in [\n']$.
\end{compactitem} \label{line:psi:bob}

\bigskip

\Statex \hspace{-\algorithmicindent} {\bf Simulate $\prot$ on $G$ assuming first message is $\Pi_1$:} \vspace{5pt}

\bigskip 

\State Alice (respectively, Bob) simulates the protocol $\prot$ on input $G$ from Bob's (resp. Alice's) perspective, starting from the second round assuming that the message $\Pi_1$ was sent in the first round.  \label{line:psi:comm2}

\end{algorithmic}
\end{algorithm}

We claim that the protocol $\psi_{\prot, \Y}$ communicates at most $C$ bits in at most $(r-1)$ rounds. Indeed, the communication is at most $C$ bits as the only lines where Alice and Bob communicate is \autoref{line:psi:comm1} and \autoref{line:psi:comm2}, and bits sent in these lines would also be sent when $\prot$ is run on input $G$. Moreover, this communication happens in at most $(r-1)$ rounds as there are at most $(r-1)$ rounds of communication in \autoref{line:psi:comm2} and the message sent in \autoref{line:psi:comm1} can be sent in parallel with the first message sent in \autoref{line:psi:comm2}. 

This means that \Cref{lemma:reactual} follows once we show \eqref{eq:reactualyes} and \eqref{eq:reactualno}. To this end, for an $(S',c)$-nested block graph $G'$, define the event $\ext_{G'} \subseteq \supp{\dist}$ as follows:
\begin{equation}
\label{eq:ext}
\ext_{G'} := \forall i \in [\n']: G^{\star}_{(i-1)c \to ic} = G'^{\star}_i.
\end{equation}

Also, define, for an $(S',c)$-nested block graph $G'$ and a bijection $\Z: V'_{0} \to V'_{\n'}$, the random variable (over the randomness in \Cref{algo:psi}) $\left( \{\rv{E}^{\psi, \Z}_{i}(G')\}_{i \in [\n]}, \rv{\Pi}^{\psi, \Z}_1(G') \right)$ to be the edges of the graph $G$ and the message $\Pi_1$ sampled by $\psi_{\prot, \Z}$ before \autoref{line:psi:comm2} on input $G'$. Note that, as the first and the last layers of $G'$ have the same size as the first and the last layers of $G$, we can view any bijection $\Z: V'_0 \to V'_{\n'}$ as a bijection $\Z: V_0 \to V_{\n}$. We claim that:
\begin{lemma}
\label{lemma:reactualactual}
For all bijections $\Z: V_0 \to V_{\n}$, we have:
\begin{multline*}
\E_{G' \sim \dist'} \Bracket{ \tvd{ \distributions{ \{ \rv{E}_i \}_{i \in [\n]}, \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'} } }{ \distribution{ \{\rv{E}^{\psi, G'^{\star} \circ \Z^{-1}}_{i}(G')\}_{i \in [\n]}, \rv{\Pi}^{\psi, G'^{\star} \circ \Z^{-1}}_1(G') } } }\\
\leq  \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .
\end{multline*}
\end{lemma}


We defer the proof of \Cref{lemma:reactualactual} to later but use it here to finish the proof of \Cref{lemma:reactual}.  \TODO{Finish this proof}

\end{proof}


We now show \Cref{lemma:reactualactual}.

\begin{proof}[Proof of \Cref{lemma:reactualactual}]
Fix a bijection $\Z: V_0 \to V_{\n}$. For $G' \in \supp{\dist'}$, define the distributions:
\begin{equation}
\label{eq:init}
\begin{split}
\init^{\prot}_{G'} &= \distributions{ \{ \rv{E}_i \}_{i \in [\n]}, \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'} } , \\
\init^{\psi}_{G'} &= \distribution{ \{\rv{E}^{\psi, G'^{\star} \circ \Z^{-1}}_{i}(G')\}_{i \in [\n]}, \rv{\Pi}^{\psi, G'^{\star} \circ \Z^{-1}}_1(G') } .
\end{split}
\end{equation}

Using this notation, in order to show \Cref{lemma:reactualactual}, it is sufficient to show that:
\begin{equation}
\label{eq:reactualactual}
\E_{G' \sim \dist'} \Bracket{ \tvd{ \init^{\prot}_{G'} }{ \init^{\psi}_{G'} } } \leq \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .
\end{equation}
We show this using \Cref{fact_tvd_chain_rule}. Define the random variables:
\begin{compactitem}
\item $\rv{L}_{1, \ev} = \{\rv{E}_{i}\}_{i = \n - c + 1, \ev~i}^{\n}$, $\rv{L}_{1, \od} = \{\rv{E}_{i}\}_{i = \n - c + 1, \od i}^{\n}$, and $\rv{L}_{1} = (\rv{L}_{1, \od}, \rv{L}_{1, \ev})$.
\item $\rv{L}_{2, \ev} = \{\rv{E}_{(i-1)c + j}\}_{\ev~i \in [\n'], \ev~j \in [c]}$, $\rv{L}_{2, \od} = \{\rv{E}_{(i-1)c + j}\}_{\od~i \in [\n'], \od~j \in [c]}$,\\ and $\rv{L}_{2} = (\rv{L}_{2, \od}, \rv{L}_{2, \ev})$.
\item $\rv{L}_3 = \{\rv{E}_{(i-1)c + j}\}_{\ev~i \in [\n'], \od~j \in [c]}$.
\item $\rv{L}_4 = \rv{\Pi}_1$.
\item $\rv{L}_5 = \{\rv{E}_{(i-1)c + j}\}_{\od~i \in [\n'], \ev~j \in [c]}$.
\end{compactitem}
and note that both $\init^{\prot}_{G'}$ and $\init^{\psi}_{G'}$ are distributions over the tuple $(\rv{L}_{1}, \rv{L}_{2}, \rv{L}_{3}, \rv{L}_{4}, \rv{L}_{5})$. Thus, by \Cref{fact_tvd_chain_rule}, we have
\begin{multline*}
\E_{G' \sim \dist'} \Bracket{ \tvd{ \init^{\prot}_{G'} }{ \init^{\psi}_{G'} } } \\
\leq \sum_{i = 1}^5 \E_{G' \sim \dist'} \E_{(L_1, \cdots, L_{i-1}) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{i} \mid L_1, \cdots, L_{i-1} }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{i} \mid L_1, \cdots, L_{i-1} }{ \init^{\psi}_{G'} } } } ,
\end{multline*}
and \eqref{eq:reactualactual} follows once we show \Cref{claim:reactualactual1,claim:reactualactual2,claim:reactualactual3,claim:reactualactual4,claim:reactualactual5} below:

\begin{claim}
\label{claim:reactualactual1}
We have:
\[
\E_{G' \sim \dist'} \Bracket{ \tvd{ \distributions{ \rv{L}_{1} }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{1} }{ \init^{\psi}_{G'} } } } = 0 .
\]
\end{claim}
\begin{proof}
This claim holds for all $G'$\footnote{Observe that $\tvd{d_1}{d_2}$ is non-negative for all distributions $d_1, d_2$. Thus, the expectation is $0$ if and only if it is $0$ almost surely.} Fix $G'$ and consider first the distribution $\distributions{ \rv{L}_{1} }{ \init^{\prot}_{G'} }$. By definition, this is the distribution of the edges $\rv{L}_{1}$ of a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}$. Due to the conditioning, this is simply the uniform distribution over the edges $\{E_{i}\}_{i = \n - c + 1}^{\n}$ conditioned on $G^{\star}_{\n - c \to \n} = \hat{\Y} \circ \Z \circ \paren{G'^{\star}}^{-1}$.

Now, consider the distribution $\distributions{ \rv{L}_{1} }{ \init^{\psi}_{G'} }$. By \autoref{line:psi:last}, this is just the uniform distribution on $\{E_{i}\}_{i = \n - c + 1}^{\n}$ conditioned on $G^{\star}_{\n - c \to \n} = \hat{\Y} \circ \Z \circ \paren{G'^{\star}}^{-1}$. Thus, the two distributions are identical.
\end{proof}



\begin{claim}
\label{claim:reactualactual2}
We have:
\[
\E_{G' \sim \dist'} \E_{L_1 \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{2} \mid L_1 }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{2} \mid L_1 }{ \init^{\psi}_{G'} } } } = 0 .
\]
\end{claim}
\begin{proof}
This claim holds for all $G'$ and $L_1$. Fix $G'$ and $L_1$ and consider first the distribution $\distributions{ \rv{L}_{2} \mid L_1 }{ \init^{\prot}_{G'} }$. By definition, this is just the marginal distribution of the edges $L_2$ of a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_1$. Due to the fact that for all $i \in [\n']$, there exists a $j$ such that $E_{(i-1)c + j}$ is not sampled and that all the layers in between $V_{(i-1)c}$ and $V_{ic}$ are of the same size and larger than $V_{(i-1)c}$ and $V_{ic}$, this distribution is just the uniform distribution over all possible values of $L_2$. 

Now, consider the distribution $\distributions{ \rv{L}_{2} \mid L_1 }{ \init^{\psi}_{G'} }$. By \autoref{line:psi:even}, this is also the uniform distribution over all possible values of $L_2$, and thus identical.
\end{proof}



\begin{claim}
\label{claim:reactualactual3}
We have:
\[
\E_{G' \sim \dist'} \E_{(L_1, L_2) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{3} \mid L_1, L_2 }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{3} \mid L_1, L_2 }{ \init^{\psi}_{G'} } } } = 0 .
\]
\end{claim}
\begin{proof}
The claim holds for all $G', L_1, L_2$. Fix $G, L_1, L_2$ and consider first the distribution $\distributions{ \rv{L}_{3} \mid L_1, L_2 }{ \init^{\prot}_{G'} }$. By definition, this is just the marginal distribution of the edges $L_3 = \{E_{(i-1)c + j}\}_{\ev~i \in [\n'], \od~j \in [c]}$ of a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_1, L_2$. Observe first that, conditioned on $\ext_{G'}$, the random variable $\rv{L}_{3}$ is independent of $\rv{L}_{1}$ and $\rv{L}_{2, \od}$. Thus, the distribution $\distributions{ \rv{L}_{3} \mid L_1, L_2 }{ \init^{\prot}_{G'} }$ is the marginal distribution of $L_3$ in a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_{2, \ev}$ and moreover, the latter is just the uniform distribution over all possible values of $L_3$ conditioned on $L_{2, \ev}$ and $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all even $i \in [\n']$. 

Now, consider the distribution $\distributions{ \rv{L}_{3} \mid L_1, L_2 }{ \init^{\psi}_{G'} }$. By \autoref{line:psi:alice1}, this is also the uniform distribution over all possible values of $L_3$ conditioned on  $L_{2, \ev}$ and $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all even $i \in [\n']$, and the two distributions are identical.
\end{proof}

\TODO{Exactly how does $\ext$ break correlation? is it independent across all blocks?}

\begin{claim}
\label{claim:reactualactual4}
We have:
\begin{multline*}
\E_{G' \sim \dist'} \E_{(L_1, L_2, L_3) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\psi}_{G'} } } } \\
\leq \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)} .
\end{multline*}
\end{claim}
\begin{proof}
Consider first the distribution $\distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} }$. By definition, this is the distribution of the first message $\Pi_1$ sent by the protocol $\prot$ when run with a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_1, L_2, L_3$ as input. As the protocol $\prot$ is deterministic, we have that $\Pi_1$ is a function of $(L_{1, \ev}, L_{2, \ev}, L_5)$. As, conditioned on $\ext_{G'}, L_{1, \ev}, L_2$, the random variable $\rv{L}_5$ is independent of the random variables  $\rv{L}_{1, \od}, \rv{L}_3$, we have that the distribution $\distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} }$ is the same as the distribution of the first message $\Pi_1$ sent by the protocol $\prot$ when run with a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_{1, \ev}, L_2$ as input. 

Next, use the fact that the marginal distribution of $\rv{L}_5$ is the same in $G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'}, L_{1, \ev}, L_2$ and $G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2$ to conclude that the distribution $\distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} }$ is the same as the distribution of the first message $\Pi_1$ sent by the protocol $\prot$ when run with a graph $G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2$ as input. 


For convenience, henceforth, we break the event $\ext_{G'}$ into two events $\ext_{G'} = \ext_{G', \ev} \wedge \ext_{G', \od}$:
\[
\ext_{G', \ev} := \forall~\ev~i \in [\n']: G^{\star}_{(i-1)c \to ic} = G'^{\star}_i \quad\text{and}\quad \ext_{G', \od} := \forall~\od~i \in [\n']: G^{\star}_{(i-1)c \to ic} = G'^{\star}_i.
\]
Observe from \autoref{line:psi:alice2} that the distribution $\distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\psi}_{G'} }$ is the same as the distribution $\distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G', \ev}, L_{1, \ev}, L_2 }$. We get:
\begin{align*}
&\E_{G' \sim \dist'} \E_{(L_1, L_2, L_3) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\psi}_{G'} } } } \\
&= \E_{G' \sim \dist'} \E_{(L_1, L_2, L_3) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2 } }{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G', \ev}, L_{1, \ev}, L_2 } } } \\
&= \E_{\substack{G' \sim \dist' \\ (L_{1, \ev}, L_2) \sim \init^{\prot}_{G'}}} \Bracket{ \tvd{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2 } }{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G', \ev}, L_{1, \ev}, L_2 } } } \\
&\leq \E_{\substack{G' \sim \dist' \\ (L_{1, \ev}, L_2) \sim \init^{\prot}_{G'}}} \Bracket{ \sqrt{ \frac{1}{2} \cdot \kl{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2 } }{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G', \ev}, L_{1, \ev}, L_2 } } } } \tag{\Cref{prelim-fact:pinskers}} \\
&\leq \sqrt{ \frac{1}{2} \cdot \E_{\substack{G' \sim \dist' \\ (L_{1, \ev}, L_2) \sim \init^{\prot}_{G'}}} \Bracket{ \kl{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G'}, L_{1, \ev}, L_2 } }{ \distributions{ \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y}} \mid \ext_{G', \ev}, L_{1, \ev}, L_2 } } } } \tag{Concavity of $\sqrt{\cdot}$} .
\end{align*}
To continue, note that, by symmetry, sampling $G' \sim \dist'$  is the same as sampling $G \sim \dist^{\hat{\Y}}$ and setting $G'$ to be the unique set of edges satisfying $G^{\star}_{(i-1)c \to ic} = G'^{\star}_i$ for all $i \in [\n']$. Thus, sampling $G' \sim \dist'$ and then sampling $(L_{1, \ev}, L_2) \sim \init^{\prot}_{G'}$ is the same as sampling $G_1 \sim \dist^{\hat{\Y}}$ and then sampling edges $(L_{1, \ev}, L_2)$ of a graph $G \sim \dist^{\hat{\Y} \circ \Z} \mid \{G^{\star}_{(i-1)c \to ic}\}_{i \in [\n']} = \{G^{\star}_{1, (i-1)c \to ic}\}_{i \in [\n']}$ by the definition of $\init^{\prot}_{G'}$ and \Cref{eq:ext}.

As we do not sample $L_{1, \od}$, the latter is the same as sampling edges $(L_{1, \ev}, L_2)$ of a graph $G \sim \dist^{\hat{\Y}} \mid \{G^{\star}_{(i-1)c \to ic}\}_{i \in [\n']} = \{G^{\star}_{1, (i-1)c \to ic}\}_{i \in [\n']}$ which makes the overall procedure just sampling the random variables $(\{\rv{G}^{\star}_{(i-1)c \to ic}\}_{i \in [\n']}, \rv{L}_{1, \ev}, \rv{L}_{2}) \sim \dist^{\hat{\Y}}$. Using the notation,
\[
\Upsilon = (\{G^{\star}_{(i-1)c \to ic}\}_{\od~i \in [\n']}, \Upsilon_{\ev} ) \quad\text{where}\quad \Upsilon_{\ev} = (\{G^{\star}_{(i-1)c \to ic}\}_{\ev~i \in [\n']}, L_{1, \ev}, L_{2} ) ,
\]
we get:
\begin{align*}
&\E_{G' \sim \dist'} \E_{(L_1, L_2, L_3) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{4} \mid L_1, L_2, L_3 }{ \init^{\psi}_{G'} } } } \\
&\hspace{1cm}\leq \sqrt{ \frac{1}{2} \cdot \E_{\Upsilon \sim \dist^{\hat{\Y}}} \Bracket{ \kl{ \distributions{ \rv{\Pi}_1(G) \mid \Upsilon }{ G \sim \dist^{\hat{\Y}} } }{ \distributions{ \rv{\Pi}_1(G) \mid \Upsilon_{\ev} }{ G \sim \dist^{\hat{\Y}} } } } } \\
&\hspace{1cm}\leq \sqrt{ \frac{1}{2} \cdot \mi{ \rv{\Pi}_1(G) }{\{\rv{G}^{\star}_{(i-1)c \to ic}\}_{\od~i \in [\n']} \mid \rv{\Upsilon}_{\ev} } } \tag{\Cref{prelim-fact:kl-info}} \\
&\hspace{1cm}\leq \sqrt{ \frac{1}{2} \cdot \sum_{\od~i \in [\n']} \mi{ \rv{\Pi}_1(G) }{ \rv{G}^{\star}_{(i-1)c \to ic} \mid \rv{\Upsilon}_{\ev}, \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\od~i' < i \in [\n']} } } \tag{\Cref{fact:it-facts}, \Cref{part:chain-rule}} .
\end{align*}
Thus, the claim follows once we show that, for all $\od~i \in [\n']$, we have
\begin{equation}
\label{eq:reactualactual1}
\mi{ \rv{\Pi}_1(G) }{ \rv{G}^{\star}_{(i-1)c \to ic} \mid \rv{\Upsilon}_{\ev}, \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\od~i' < i \in [\n']} } \leq \Phi(s_{\card{S}},s_{\card{S'}},c,C) .
\end{equation}
\Cref{eq:reactualactual1} is true because:
\begin{align*}
&\mi{ \rv{\Pi}_1(G) }{ \rv{G}^{\star}_{(i-1)c \to ic} \mid \rv{\Upsilon}_{\ev}, \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\od~i' < i \in [\n']} } \\
&\hspace{1cm}= \mi{ \rv{\Pi}_1(G) }{ \rv{G}^{\star}_{(i-1)c \to ic} \mid \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\ev~i' \in [\n']}, \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\od~i' < i \in [\n']}, \rv{L}_{1, \ev}, \rv{L}_{2} } \tag{Definition of $\Upsilon_{\ev}$} \\
&\hspace{1cm}= \mi{ \rv{\Pi}_1(G) }{ \rv{G}^{\star}_{(i-1)c \to ic} \mid \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\ev~i' \in [\n']}, \{\rv{G}^{\star}_{(i'-1)c \to i'c}\}_{\od~i' < i \in [\n']}, \rv{L}_{1, \ev}, \rv{L}_{2} } \tag{\Cref{prelim-prop:info-increase}} \\
\end{align*}

\TODO{Start here}

\end{proof}


\begin{claim}
\label{claim:reactualactual5}
We have:
\[
\E_{G' \sim \dist'} \E_{(L_1, \cdots, L_{i-1}) \sim \init^{\prot}_{G'}} \Bracket{ \tvd{ \distributions{ \rv{L}_{i} \mid L_1, \cdots, L_{i-1} }{ \init^{\prot}_{G'} } }{ \distributions{ \rv{L}_{i} \mid L_1, \cdots, L_{i-1} }{ \init^{\psi}_{G'} } } } = 0 .
\]
\end{claim}
\begin{proof}
\end{proof}


\end{proof}









\vspace{5cm}





Using \Cref{lemma:tvdtriangle} on \Cref{lemma:reactualactual}, we have for all $\Z$ that:
\begin{multline*}
\tvd{ \distributions{ \{ \rv{E}_i \}_{i \in [\n]}, \rv{\Pi}_1(G) }{ G' \sim \dist', G \sim \dist^{\hat{\Y} \circ \Z} \mid \ext_{G'} } }{ \distributions{ \{\rv{E}^{\psi, G'^{\star} \circ \Z^{-1}}_i(G')\}_{i \in [\n]}, \rv{\Pi}^{\psi, G'^{\star} \circ \Z^{-1}}_1(G') }{ G' \sim \dist' } } \\
\leq  \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)}    .
\end{multline*}
By symmetry, we have
\begin{multline*}
\tvd{ \distributions{ \{ \rv{E}_i \}_{i \in [\n]}, \rv{\Pi}_1(G) }{ G \sim \dist^{\hat{\Y} \circ \Z} } }{ \distributions{ \{\rv{E}^{\psi, \Y}_i(G')\}_{i \in [\n]}, \rv{\Pi}^{\psi, \Y}_1(G') }{ \Y \sim \disty, G' \sim \dist'^{\Y \circ \Z} } } \\
\leq  \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)}    .
\end{multline*}

As the protocol $\psi_{\prot, \Y}$ merely simulates the protocol $\prot$ (from the second message onwards) after sampling the tuple $\left( \{E^{\psi, \Y}_i(G')\}_{i \in [\n]}, \Pi^{\psi, \Y}_1(G') \right)$ and the protocol $\prot$ is deterministic, we have that:
\[
\tvd{ \distributions{ \rv{O}^{\prot}(G) }{ G \sim \dist^{\hat{\Y} \circ \Z} } }{ \distributions{ \rv{O}^{\psi_{\prot, \Y}}(G') }{ \Y \sim \disty, G' \sim \dist'^{\Y \circ \Z} } } \leq  \frac{1}{2} \cdot \sqrt{\n' \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)}    .
\]
Plugging in $Z = $ the `identity' bijection and $\Z = \Delta$ finishes the proof of \Cref{lemma:reactual}.

















\newcommand{\ths}[1]{\relax\ifmmode{}_\theta#1\else$_\theta$#1\fi\relax}
\newcommand{\pis}[1]{\relax\ifmmode{}_\pi#1\else$_\pi$#1\fi\relax}





Fix a matching $\Pdelta$, for technical reasons, we will only consider pairs $(\Pyes,\Pno)$ such that $\Pyes=\Pdelta\circ\Pno$.
In fact, we can even replace the the $\max$ on the LHS with with an average value, i.e.,
\[
	\E_{P} [\adv(m,c,r-1, C, P, \Pdelta^{-1}\circ P)]\geq \max_{\stackrel{\Pyes,\Pno:}{\Pyes=\Pdelta\circ\Pno}} \{\adv(m,c,r, C, \Pyes, \Pno)\}-\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)},
\]
where $P$ on the LHS is sampled uniformly at random.
By the fact that the expectation is at most the maximum, and taking a $\max$ over $\Pdelta$ on both sides, the above inequality implies the lemma.
In the following, let us focus only on this inequality.

Consider the LHS, since $P$ is a random matching, both distributions in the definition of $\adv$ are marginally the uniform distribution $\dist_{r-1}$.
Thus, it is helpful to view the left-hand-side as how well the players can distinguish the following two cases:
\begin{compactenum}[(a)]
	\item given a \emph{uniformly random} $G$ and a matching $P=\Pstar(G)$;
	\item given a \emph{uniformly random} $G$ and a matching $P=\Pdelta\circ\Pstar(G)$ (i.e., the final matching is $\Pdelta^{-1}\circ P$).
\end{compactenum}

Therefore, to prove the lemma, we are going to show that for any $r$-round protocol $\pi$ and any pair $\Pyes,\Pno$ such that $\Pyes=\Pdelta\circ\Pno$, we can use it to construct an $(r-1)$-round protocol $\theta$ whose the total variation distance between case (a) and case (b) above is at least
\[
	\tvd{\distributions{\rv \Pi(G)}{G\sim\dist_r\mid \rv \Pstar(G)=\Pyes}}{\distributions{\rv \Pi(G)}{G\sim\dist_r\mid \rv \Pstar(G)=\Pno}}-\sqrt{k_{c,r-1}\cdot \Phi(m,c,\norm{\pi})}.
\]

To this end, recall that a graph sampled from $\dist_r$ has $k_{c,r}$ matchings (and hence $k_{c,r}+1$ layers) for $k_{c,r}=2c\cdot (k_{c,r-1}+1)$.
Thus, we view a graph with $k_{c,r}$ matchings as $k_{c,r-1}+1$ \emph{blocks} of size $2c$.
More formally, we define the blocks as follows (see also~\Cref{fig_1}).

\begin{definition}[\textbf{Block}]\label{def:block}
A \emph{block} $\block{i} = (\Vb{i},\Eb{i})$ is the following subgraph: 
\begin{enumerate}[label=$(\roman*)$]
	\item $\Vb{i} := \Vb{i}_0 \sqcup \Vb{i}_1 \sqcup \Vb{i}_2 \sqcup \ldots \sqcup \Vb{i}_{2c-1} \sqcup \Vb{i}_{2c}$, where each  $\Vb{i}_j$ is a \emph{layer} and is of size $m$. 
	% We denote $\Sb{i} := \Ub{i}_0$ as the \emph{starting layer} and $\Tb{i} := \Ub{i}_{2c}$ as the \emph{target layer}. 
	\item $\Eb{i} := \Mb{i}_1 \sqcup \Mb{i}_2 \sqcup \ldots \sqcup \Mb{i}_{2c}$, where each $\Mb{i}_j$ is a perfect matching between $\Vb{i}_{j-1}$ and $\Vb{i}_j$. 
\end{enumerate}
For any block $\block{i}$, we define its \emph{block-matching} $\Pb{i}$ as $\Mb{i}_{2c}\circ \Mb{i}_{2c-1}\circ\cdots \Mb{i}_1$, i.e., the composition of all matchings in the block.
\end{definition}

\begin{figure}
\input{Files/fig-re.tex}
\caption{The upper graph is divided into five \emph{blocks} of two matchings. The red matchings are given to Alice, while the blue matchings are Bob's inputs. The lower graph is the corresponding \emph{block matchings}.}\label{fig_1}
\end{figure}

Therefore, the $k_{c,r}$ matchings can be viewed as $k_{c,r-1}+1$ consecutive blocks with $\Vb{i}_{2c}=\Vb{i+1}_0$.
Equivalently, this is a relabeling of the matchings such that $\Mb{i}_j$ is $M_{2c\cdot i+j}$ for $i=0,\ldots,k_{c,r-1}$ and $j=1,\ldots,2c$.
Block $\block{0}$ is a special block, which we will discuss later.
For the remaining $k_{c,r-1}$ blocks, their block matchings can be viewed as a $(m,k_{c,r-1})$-layered graph.
This allows the players in protocol $\theta$ to use $\pi$.
% In the $(r-1)$-round protocol $\theta$, given an instance sampled from $\dist_{r-1}$ (together with a matching $\Pstar$), we are going to view it as the graph of \emph{block matchings} of a $(m,k_{c,r})$-layered graph.
More specifically, given an instance sampled from $\dist_{r-1}$ (together with a matching $ P$), the two players are going to collaboratively sample (using both public and private randomness but \emph{no} communication) a $(m, k_{c,r})$-layer graph $G$ whose $i$-th \emph{block matching} is equal to the $i$-th matching of the input graph.
Moreover, the sampling algorithm will guarantee that 
\begin{enumerate}
	\item if $P$ is the final matching of the input graph (case (a) above), then $G$ is a graph with final matching $\Pyes$; 
	\item if $P$ is $\Pdelta$ composed with the final matching of the input graph (case (b) above), then $G$ is a graph with final matching $\Pno$.
\end{enumerate}
Thus, if $\pi$ can distinguish the final matching being $\Pyes$ or $\Pno$, the players can then simulate $\pi$ to distinguish between the above two cases.
The most important feature of our sampling procedure is that it simultaneously \emph{publicly} samples $\Pi_1$, the \emph{first message} of $\pi$.
Therefore, the players do not only know their parts of $G$ to simulate $\pi$, but they also get to know the first message of the protocol \emph{with no communication}, which allows them to start the simulate directly from the second round, and consequently, reduces the number of rounds by one.

\paragraph{Protocol $\theta$.}

To avoid ambiguity, we will \emph{left-subscript} all variables to indicate whether they are associated with $\theta$ or $\pi$.
For example, the players are denoted by \ths{Alice} and \ths{Bob}, while the players of $\pi$ that they simulate are \pis{Alice} and \pis{Bob}.
The input graph to $\theta$ is $\ths{G}$, the input graph to $\pi$ that the players generate is $\pis{G}$.

We use $\dist_{\pi\mid \Pyes}$ to denote the joint distribution of $(\rv M_A, \rv M_B, \rv \Pi)$ where the input matchings $(\rv M_A, \rv M_B)$ is from a graph following the distribution $\dist_r$ \emph{conditioned on} the final matching being $\Pyes$, and $\rv \Pi$ is the transcript of protocol $\pi$ on $(\rv M_A, \rv M_B)$.
Similarly, we use $\dist_{\pi\mid \Pno}$ to denote the joint distribution of $(\rv M_A, \rv M_B, \rv \Pi)$ when $(\rv M_A, \rv M_B)$ is from a graph following $\dist_r$ conditioned on the final matching being $\Pno$, and $\rv \Pi$ is its transcript.

\begin{tbox}
\textbf{Protocol $\theta$.}

\medskip

Given as input $\ths{G}$ consisting of $(\ths{M_1},\ldots,\ths{M_{k_{c,r-1}}})$ and a matching $ P$, \ths{Alice} receives $\{\ths{M}_i\}_{\textrm{even }i}$ and $ P$, \ths{Bob} receives $\{\ths{M}_i\}_{\textrm{odd }i}$ and $ P$, they do as follows:
\begin{enumerate}[label=$(\roman*)$]
	\item ({\bf publicly}) sample uniformly random $\pis{\Mb{0}_j}$ for all $j$ conditioned on $P\circ\pis{\Pb{0}}=\Pyes$;
	\item ({\bf publicly}) sample uniformly random $\pis{\Mb{i}_j}$ for all $(i, j)$ with the \emph{same parity} and $i\geq1$ (i.e., $i,j$ both odd, or $i,j$ both even);
	\item ({\bf publicly}) sample $\Pi_1$, the first message of $\pi$, from distribution $\dist_{\pi\mid \Pyes}$ \emph{conditioned on} $\rv \Mb^{0}_j=\pis{\Mb{0}_j}$ for all $j$ and $\rv M^i_j=\pis{\Mb{i}_j}$ for all $(i, j)$ with the \emph{same parity} and $i\geq 1$;
	\item \ths{Bob} ({\bf privately}) samples $\pis{\Mb{i}_j}$ for all odd $i$ and even $j$ according to $\dist_{\pi\mid \Pyes}$, \emph{conditioned on}
	\begin{compactitem}
		\item $\rv\Pi_1=\Pi_1$,
		\item $\rv \Mb^{0}_j=\pis{\Mb{0}_j}$ for all $j$,
		\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity and $i\geq 1$, and
		\item $\rv P^{i}=\ths{M_i}$ for all odd $i$;
	\end{compactitem}
	\item \ths{Alice} ({\bf privately}) samples $\pis{\Mb{i}_j}$ for all even $i\geq 2$ and odd $j$ according to $\dist_{\pi\mid \Pyes}$, \emph{conditioned on}
	\begin{compactitem}
		\item $\rv\Pi_1=\Pi_1$,
		\item $\rv \Mb^{0}_j=\pis{\Mb{0}_j}$ for all $j$,
		\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity and $i\geq 1$, and
		\item $\rv P^{i}=\ths{M_i}$ for all even $i\geq 2$;
	\end{compactitem}
	\item \ths{Alice} simulates \pis{Bob} with input $\pis{M_A}=\{\pis{\Mb{i}_j}\}_{i, \textrm{odd }j}$, \\
	\ths{Bob} simulates \pis{Alice} with input $\pis{M_B}=\{\pis{\Mb{i}_j}\}_{i, \textrm{even }j}$, \\
	starting from the second round of $\pi$ with $\Pi_1$ being the first round; \\
	\ths{Alice} includes $\Pi_1$ in her first message.
\end{enumerate} 
\end{tbox}

The following lemma and corollary state the crucial properties of the protocol.
\begin{lemma}\label{lem_th_dist_pstar}
	For a uniformly random $ P$, and $\ths{G}\sim \dist_{r-1}\mid \rv\Pstar(G)= P$, the joint distribution of
	\[
		(\pis{\rv M_A}, \pis{\rv M_B}, \rv \Pi_1)
	\]
	generated by $\theta$ (over the randomness of both $ P$ and $\ths{G}$) and the joint distribution of
	\[
		(\rv M_A,\rv M_B,\rv \Pi_1)
	\]
	from $\dist_{\pi\mid \Pyes}$ have total variation distance at most 
	\[
		\frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)},
	\]
	where $\Phi(m,c,C)$ is defined as in \Cref{lem_one_round_joint_unif}.
\end{lemma}
\begin{corollary}\label{cor_th_dist_pstar}
	For a uniformly random $ P$, if $\ths{G}\sim \dist_{r-1}\mid \rv\Pstar(G)= \Pdelta^{-1}\circ P$, the joint distribution of
	\[
		(\pis{\rv M_A}, \pis{\rv M_B}, \rv \Pi_1)
	\]
	generated by $\theta$ (over the randomness of both $ P$ and $\ths{G}$) and the joint distribution of
	\[
		(\rv M_A,\rv M_B,\rv \Pi_1)
	\]
	from $\dist_{\pi\mid \Pno}$ have total variation distance at most 
	\[
		\frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)}.
	\]
\end{corollary}
The proof of the lemma is deferred to the next subsection.
We first show that it implies \Cref{cor_th_dist_pstar}.
\begin{proof}[Proof of~\Cref{cor_th_dist_pstar}]
	First observe that in step (iii), (iv) and (v), the marginal distributions of $\dist_{\pi\mid \Pyes}$ used by the protocol \emph{does not} depend on the value of $\Pyes$.
	In particular, they are identical to the corresponding marginals from $\dist_{\pi\mid\Pno}$.
	To see this, for step (iii), $\Pi_1$ is a function of $\Mb{i}_j$ for all even $j$.
	Given the conditions, the marginal distribution of all \emph{remaining} $\Mb{i}_j$ for even $j$ is uniform and independent.
	For step (iv), given the conditions, these matchings determine both $\Pi_1$ and block matchings for odd $i$.
	Thus, the marginal distribution is simply the uniform distribution conditioned on the block matchings and $\Pi_1$.
	For step (v), it is similar to step (iv), the matchings determine the block matching for all even $i$.
	The marginal is uniform conditioned on the block matchings.

	Next, when $P$ is $\Pdelta\circ\Pstar(G)$, by the fact that $\Pyes=\Pdelta\circ\Pno$, the condition in step (i) translates to $\pis{P^{0}}=(\Pstar(G))^{-1}\circ\Pno$.
	Thus, by changing $\Pyes$ to $\Pno$ in the entire protocol and giving $\Pstar(G)$ to the players, the behavior of the protocol remains the same.
	In particular, the marginal distribution of $(\pis{\rv M_A},\pis{\rv M_B},\pis{\rv \Pi_1})$ remains the same.
	We prove the corollary by applying \Cref{lem_th_dist_pstar} for $\Pno$.
\end{proof}

\begin{proof}[Proof of~\Cref{lem:round-elimination}]
	Fix $\Pyes,\Pno$ and $\Pdelta$ such that $\Pyes=\Pdelta\circ\Pno$, and any $r$-round protocol $\pi$ with communication cost at most $C$.
	It suffices to show that the LHS is at least
	\begin{equation}\label{eqn_round_elim_rhs}
		\tvd{\distributions{\rv \Pi(G)}{\dist_{\pi\mid\Pyes}}}{\distributions{\rv \Pi(G)}{\pi\mid\Pno}}-\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)}.
	\end{equation}
	To this end, note that $\theta$ first generates (with no communication) an input pair $(\pis{M_{\even}}, \pis{M_{\odd}})$ and first message $\Pi_1$.
	Then the players start the communication by simulating protocol $\pi$ from the second round (and including $\Pi_1$ in its first message).
	Clearly, $\theta$ has $r-1$ rounds and communication cost at most $C$.
	We will show that $\theta$ has
	\begin{equation}\label{eqn_round_elim_lhs}
		\E_{ P}\tvd{\distributions{\rv \Theta(G,  P)}{G\sim\dist_r\mid \rv \Pstar(G)=  P}}{\distributions{\rv \Theta(G,  P)}{G\sim\dist_r\mid \rv \Pstar(G)=  \Pdelta^{-1}\circ P}}\geq \eqref{eqn_round_elim_rhs},
	\end{equation}
	where $\Theta(G,  P)$ is the transcript of $\Theta$ on input $G$ and $ P$.

	To prove \eqref{eqn_round_elim_lhs}, observe that once $\theta$ has generated $(\pis{M_{\even}}, \pis{M_{\odd}})$ and $\Pi_1$, it only simulates $\pi$ from there, and has a determined transcript (or a fixed distribution of transcript if $\pi$ is randomized).
	Therefore, the first distribution in \eqref{eqn_round_elim_lhs} is very close to $\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pyes}}$, since
	\begin{align*}
		&\, \E_{ P}\tvd{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)=  P}}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pyes}}} \nonumber\\
		&\leq \E_{ P}\tvd{\distributions{\pis{\rv M_{\even}}, \pis{\rv M_{\odd}}, \rv \Pi_1}{G\sim\dist_r\mid \rv \Pstar(G)=  P}}{\distributions{\rv M_{\even}, \rv M_{\odd}, \rv \Pi_1}{\dist_{\pi\mid \Pyes}}} \nonumber\\
		&\leq \frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)}, 
	\end{align*}
	where the last inequality is by \Cref{lem_th_dist_pstar}.
	Similarly, the second distribution in \eqref{eqn_round_elim_lhs} is very close to $\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pno}}$: 
	\[
		\E_{ P}\tvd{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)=  \Pdelta^{-1}\circ P }}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pno}}} \leq \frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)},
	\]
	by \Cref{cor_th_dist_pstar}.
	Finally, by triangle inequality,
	\begin{align*}
		&\, \E_{ P}\tvd{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)=  P}}{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)=   \Pdelta^{-1}\circ P}} \\
		&\geq \E_{ P}\tvd{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pyes}}}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pno}}} \\
		&\quad\quad -\E_{ P}\tvd{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)=  P}}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pyes}}}\\
		&\quad\quad -\E_{ P}\tvd{\distributions{\rv \Theta(G, P)}{G\sim\dist_r\mid \rv \Pstar(G)= \Pdelta^{-1}\circ P}}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pno}}} \\
		&\geq \E_{P}\tvd{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pyes}}}{\distributions{\rv \Pi(G)}{\dist_{\pi\mid \Pno}}} -\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)}.
	\end{align*}
	This proves Equation~\eqref{eqn_round_elim_lhs}.
	Since it holds for all $\pi$ and all $\Pyes, \Pno$ and $\Pdelta$ such that $\Pyes=\Pdelta\circ \Pno$, we prove the lemma.
\end{proof}

\subsection{Proof of \Cref{lem_th_dist_pstar}}
Given input matchings $\ths{M_1},\ldots,\ths{M_{k_{c,r-1}}}$, \ths{Alice} and \ths{Bob} sample a graph $\pis{G}$ with $k_{c,r}$ matchings such that $\pis{\Pb{i}}$, the $i$-th block matching of $\pis{G}$, is the $i$-th input matching $\ths{M_i}$.
In the following, we analyze the protocol step-by-step, and show that each component the players sample is close to corresponding (conditional) marginal distribution from $\dist_{\pi\mid\Pyes}$.
\paragraph{Inputs.} Since $P$ is uniform, the marginal distribution of $$\ths{\rv M_1},\ldots,\ths{\rv M_{k_{c,r-1}}}$$ is all uniform and independent.
Thus, they are identically distributed as $$\rv\Pb^{1},\ldots,\rv\Pb^{k_{c,r-1}}$$ from $\dist_{\pi\mid\Pyes}$.
The goal of the players is to sample a graph with $k_{c,r}$ matchings and first message $\Pi_1$ from $\pi$ on this graph.
The ``correct'' distribution that an ideal procedure would sample from is
\[
	\{\rv\Mb^{i}_j\}_{0\leq i\leq k_{c,r-1},1\leq j\leq 2c}, \Pi_1\mid (\rv\Pb^{1}=\ths{M_1},\ldots,\rv\Pb^{k_{c,r-1}}=\ths{M_{k_{c,r-1}}})
\]
according to $\dist_{\pi\mid\Pyes}$. We now examine how our sampling process ``simulates'' this ideal distribution. 

\paragraph{Step (i).} $\pis M^0_j$ for all $j$ are sampled uniformly conditioned on $\pis P^0=P^{-1}\circ \Pyes$, and $P=\ths M_{k_{c,r-1}}\circ\cdots\circ \ths M_1$.
Similarly, in $\dist_{\pi\mid\Pyes}$, $\{\pis M^0_j\}$ are uniform conditioned on $\Pb{k_{c,r-1}}\circ\cdots\circ \Pb{1}\circ \Pb{0}=\Pyes$.
Thus, the conditional distribution
\[
	\{\pis{\rv M^0_j}\}_j \,\mid \, \ths{\rv M_1}=\ths{M_1},\ldots,\ths{\rv M_{k_{c,r-1}}}=\ths M_{k_{c,r-1}}
\]
and
\[
	\{{\rv M^0_j}\}_j \,\mid \, \rv \Pb^{1}=\ths{M_1},\ldots,\rv \Pb^{k_{c,r-1}}=\ths{M_{k_{c,r-1}}}
\]
are identical.
\paragraph{Step (ii).} Conditioned on $\Pb{1},\ldots,\Pb{k_{c,r-1}},\{\pis{M^0_j}\}_j$, the set of matchings $\Mb{i}_j$ for all $i,j$ with the same parity is uniform and independent.
Thus,
\[
	\pis {\rv\Mb^{i}_j}\textrm{ for $i,j$ with same parity} \,\mid\, \ths{\rv M_1},\ldots,\ths{\rv M_{k_{c,r-1}}}, \{\pis{\rv M^0_j}\}_j 
\]
and
\[
	\rv\Mb^{i}_j\textrm{ for $i,j$ with same parity} \,\mid\, \rv\Pb^{1},\ldots,\rv\Pb^{k_{c,r-1}}, \{\rv M^0_j\}_j 
\]
are again identically distributed.
\paragraph{Step (iii).} The protocol then samples $\Pi_1$ according to $\dist_{\pi\mid \Pyes}$ conditioned on 
\begin{compactitem}
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^i_j=\pis{\Mb{i}_j}$ for all $(i, j)$ with the \emph{same parity} and $i\geq 1$.
\end{compactitem}
The ``correct'' distribution that the players should sample from is $\Pi_1$ conditioned on all variables that have been sampled so far:
\begin{compactitem}
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^i_j=\pis{\Mb{i}_j}$ for all $(i, j)$ with the \emph{same parity} and $i\geq 1$, and
	\item $\rv \Pb^{1}=\ths{M_1},\ldots,\rv \Pb^{k_{c,r-1}}=\ths{M_{k_{c,r-1}}}$.
\end{compactitem}
The following lemma shows that they are very close.
\begin{lemma}
	For any $\Pyes$, under the distribution $\dist_{\pi\mid \Pyes}$, we have
	\[
		\mi{\rv\Pi_1}{\rv \Pb^{1},\ldots,\rv \Pb^{k_{c,r-1}}}[\{\rv M^0_j\}_j,\rv M^i_j\textrm{ for $i,j$ same parity}]\leq \frac{k_{c,r-1}}{2}\cdot \Phi(m, c, C).
	\]
\end{lemma}
\begin{proof}
	To prove the lemma, let us first temporarily remove $\rv M^0_j$ for \emph{all odd} $j$ from the condition.
	Then the marginal distribution of the other matchings are all uniform and independent.
	Also, $\rv\Pi_1$ is a function of only $\{\rv M^i_j\}_{\textrm{even }j}$.
	Then, we have
	\begin{equation}\label{eqn_lem_th_1}
		\mi{\rv\Pi_1}{\{\rv \Pb^i\}_{\textrm{even }i\geq 2}}[\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}]=0.
	\end{equation}
	This is because
	\begin{align*}
		&\,\mi{\rv\Pi_1}{\{\rv \Pb^i\}_{\textrm{even }i\geq 2}}[\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}] \\
		&\leq \mi{\{\rv M^i_j\}_{\textrm{even }j}}{\{\rv \Pb^i\}_{\textrm{even }i\geq 2}}[\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}] \\
		&=\mi{\{\rv M^i_j\}_{\textrm{odd }i, \textrm{even }j}}{\{\rv \Pb^i\}_{\textrm{even }i\geq 2}}[\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}] \\
		&=0.
	\end{align*}

	Next, consider
	\begin{equation}\label{eqn_lem_th_2}
		\mi{\rv\Pi_1}{\{\rv \Pb^i\}_{\textrm{odd }i}}[\{\rv \Pb^i\}_{\textrm{even }i\geq 2},\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}].
	\end{equation}
	By chain rule, it is equal to
	\begin{equation}\label{eqn_lem_th_3}
		\sum_{i^*=1,3,\ldots,k_{c,r-1}-1} \mi{\rv\Pi_1}{\rv \Pb^{i^*}}[\{\rv \Pb^i\}_{\textrm{odd }i<i^*},\{\rv \Pb^i\}_{\textrm{even }i\geq 2},\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}].
	\end{equation}
	Since $\rv\Pb^{i^*}$ is independent of all $\rv M^i_j$ for $i\neq i^*$ and $i\neq 0$, conditioned on all $\rv M^i_j\textrm{ for $i,j$ same parity}$ (again this is because we do not condition on $\rv M^0_j$ for odd $j$), by \Cref{prelim-prop:info-increase} and the fact that $\rv P^i$ is determined by the matchings $\rv M^i_j$, the term $i^*$ in the above sum is at most
	\[
		\mi{\rv\Pi_1}{\rv \Pb^{i^*}}[\{\rv M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j},\{\rv M^0_j\}_{\textrm{even }j},\{\rv M^{i^*}_j\}_{j\textrm{ same parity as }i^*}].
	\]
	Once we have conditioned on all inputs outside block $i^*$, the problem reduces to a one-block instance in block $i^*$.
	By a standard embedding argument and \Cref{lem_one_round_joint_unif}, 
	\begin{equation}\label{eqn_lem_th_3_5}
		\mi{\rv\Pi_1}{\rv \Pb^{i^*}}[\{\rv M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j},\{\rv M^0_j\}_{\textrm{even }j},\{\rv M^{i^*}_j\}_{j\textrm{ same parity as }i^*}]\leq\Phi(m,c,C).
	\end{equation}

	We now formalize this. Let us fix an assignment $\{M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j}, \{M^0_j\}_{\textrm{even }j}$ to variables $\{\rv M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j},\{\rv M^0_j\}_{\textrm{even }j}$ that maximizes the conditional mutual information.
	Since the matchings in block $i^*$ are independent of the condition, they are still uniform and independent.
	Now suppose two players Alice and Bob are given a $(m,2c)$-layered graph (as in the setting of \Cref{lem_one_round_joint_unif}), they simply treat this graph as block $i^*$, and use $\{M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j}, \{M^0_j\}_{\textrm{even }j}$ for the other matchings.
	Then Alice sends the first message of $\pi$ to Bob.
	The mutual information between this message and the matching of the block conditioned on Bob's input is
	\begin{align*}
		&\, \mi{\rv\Pi_1}{\rv \Pb^{i^*}}[\rv M^i_j=M^i_j\textrm{ for all } i\neq i^*,0,\rv M^0_j=M^0_j\textrm{ for all even $j$},\{\rv M^{i^*}_j\}_{j\textrm{ same parity as }i^*}] \\
		&\geq \mi{\rv\Pi_1}{\rv \Pb^{i^*}}[\{\rv M^i_j\}_{i\neq i^*\,\textrm{or}\,0,\,\textrm{all }j},\{\rv M^0_j\}_{\textrm{even }j},\{\rv M^{i^*}_j\}_{j\textrm{ same parity as }i^*}].
	\end{align*}
	On the other hand, by \Cref{lem_one_round_joint_unif}, it is also at most $\Phi(m,c,C)$.
	Thus, Equation~\eqref{eqn_lem_th_3_5} holds.

	Then by Equation~\eqref{eqn_lem_th_3}, Equation~\eqref{eqn_lem_th_2} is at most $\frac{k_{c,r-1}}{2}\cdot \Phi(m,c,C)$.
	By summing it with Equation~\eqref{eqn_lem_th_1} and applying chain rule, we have
	\[
		\mi{\rv\Pi_1}{\rv \Pb^{1},\ldots,\rv \Pb^{k_{c,r-1}}}[\{\rv M^0_j\}_{\textrm{even }j},\rv M^i_j\textrm{ for $i,j$ same parity}]\leq \frac{k_{c,r-1}}{2}\cdot \Phi(m, c, C).
	\]
	Finally, observe that conditioned on $\rv \Pb^1,\ldots,\rv\Pb^{k_{c,r-1}}$ and $\{\rv M^0_j\}_{\textrm{even }j}$, the matchings $\{\rv M^0_j\}_{\textrm{odd }j}$ are independent of $\rv \Pi_1$ and all other $\rv M^i_j$.
	% Thus, $\rv M_{k_{c,r}-1}$ is determined by $\rv \Pb^{1},\ldots,\rv \Pb^{k_{c,r-1}}$ when $\rv M_{k_{c,r}}$ is given.
	By \Cref{prelim-prop:info-decrease}, adding $\{\rv M^0_j\}_{\textrm{odd }j}$ to the condition could only decrease the mutual information, and thus,
	\[
		\mi{\rv\Pi_1}{\rv \Pb^{1},\ldots,\rv \Pb^{k_{c,r-1}}}[\{\rv M^0_j\}_{\textrm{all }j},\rv M^i_j\textrm{ for $i,j$ same parity}]\leq \frac{k_{c,r-1}}{2}\cdot \Phi(m, c, C).
	\]
	This proves the lemma.
\end{proof}
Now let us continue to analyze Step (iii), by the fact that mutual information is expected KL-divergence (\Cref{prelim-fact:kl-info}) and Pinsker's inequality (\Cref{prelim-fact:pinskers}),
\begin{align*}
	&\,\E \|\distributions{\rv \Pi_1\mid \{\rv M^0_j\}_j,{\rv \Mb^{i}_j}\textrm{ for all $(i, j)$ with the same parity}}{\dist_{\pi\mid\Pyes}}\\
	&\quad\quad-\distributions{\rv \Pi_1\mid \{\rv M^0_j\}_j,{\rv \Mb^{i}_j}\textrm{ for all $(i, j)$ with the same parity},\rv \Pb^{1},\ldots,\rv \Pb^{k_{c,r-1}}}{\dist_{\pi\mid\Pyes}}\|_{\mathrm{tvd}}\\
	&\leq\frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m, c, C)}.
\end{align*}
Note that the former is distribution used by the players, while the latter is the ``correct'' distribution.
Hence, the two have (expected) total variation distance $\frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m, c, C)}$ for step (iii).
\paragraph{Step (iv).} \ths{Bob} privately samples $\ths{M^i_j}$ for all odd $i$ and even $j$ according to $\dist_{\pi\mid \Pyes}$, from $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$ conditioned on
\begin{compactitem}
	\item $\rv\Pi_1=\Pi_1$,
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity,
	\item $\rv P^{i}=\ths{M_i}$ for {all odd} $i$.
\end{compactitem}
This is identically distributed as the ``correct'' distribution, which is $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$ conditioned on everything that has been sampled:
\begin{compactitem}
	\item $\rv\Pi_1=\Pi_1$,
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity,
	\item $\rv P^{i}=\ths{M_i}$ for {all odd} $i$, and
	\item \textbf{$\rv P^{i}=\ths{M_i}$ for all even $i\geq 2$}.
\end{compactitem}
To see this, first observe that if we do not have $\rv\Pi_1=\Pi_1$ in the condition, then both distributions are simply uniformly random $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$ conditioned on the block matchings being $\ths{M_i}$ (for all odd $i$).
That is, $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$ is independent of \textbf{$\rv P^{i}$ for all even $i\geq 2$}, given the conditions (without $\rv\Pi_1$).
On the other hand, since we have conditioned on the values of $\rv M^{i}_j$ for even $i,j$ in both distributions, and by the definition of communication protocols, $\rv \Pi_1$ is a function of \pis{Alice}'s input: $\rv \Mb^{i}_{j}$ for all even $j$.
In particular, given all other conditions, $\rv \Pi_1$ is a function of $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$.
Thus, adding $\rv \Pi_1$ to the condition does not create dependence between $\{\rv \Mb^{i}_j\}_{\textrm{odd } i, \textrm{even }j}$ and \textbf{$\rv P^{i}$ for all even $i\geq 2$}.
Therefore, the two distributions still are identical.
\paragraph{Step (v).} \ths{Alice} privately samples $\ths{M^i_j}$ for all even $i\geq 2$ and odd $j$ according to $\dist_{\pi\mid \Pyes}$, from $\{\rv \Mb^{i}_j\}$ conditioned on
\begin{compactitem}
	\item $\rv\Pi_1=\Pi_1$,
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity, 
	\item $\rv P^{i}=\ths{M_i}$ for all even $i\geq 2$.
\end{compactitem}
Similarly, this is identically distributed as the ``correct'' distribution, which is $\{\rv \Mb^{i}_j\}_{\textrm{even }i\geq 2, \textrm{odd }j}$ conditioned on everything that has been sampled:
\begin{compactitem}
	\item $\rv\Pi_1=\Pi_1$,
	\item $\rv M^0_j=\pis{M^0_j}$ for all $j$,
	\item $\rv M^{i}_j=\pis{\Mb{i}_j}$ for all $(i,j)$ with the same parity,
	\item $\rv P^{i}=\ths{M_i}$ for all even $i\geq 2$, and
	\item \textbf{$\rv P^{i}=\ths{M_i}$ for all odd $i$},
	\item \textbf{$\rv M^{i}_j=\pis{\Mb{i}_j}$ for all odd $i$ and even $j$}.
\end{compactitem}
If we do not condition on $\rv \Pi_1$, then $\{\rv \Mb^{i}_j\}_{\textrm{even }i\geq 2, \textrm{odd }j}$ are simply uniformly random matchings conditioned on the block matchings being $\ths{\Mb{i}}$ (for even $i$) in both distributions.
Therefore, $\{\rv \Mb^{i}_j\}_{\textrm{even }i\geq 2, \textrm{odd }j}$ is independent of \textbf{$\rv P^{i}$ for all odd $i$} and \textbf{$\rv M^i_j$ for all odd $i$ and even $j$}, given the other conditions (without $\rv\Pi_1$).
Next, again by the fact that $\rv\Pi_1$ is a function of $\rv M^{i}_j$ for all even $j$, $\rv\Pi_1$ is determined by $\{\rv M^{i}_j\}_{\textrm{odd }i, \textrm{even }j}$.
Thus, adding $\rv\Pi_1$ to the condition does not create dependence between $\{\rv \Mb^{i}_j\}_{\textrm{even }i\geq 2, \textrm{odd }j}$ and $\{\rv P^{i}\}_{\textrm{odd }i}$, $\{\rv M^{i}_j\}_{\textrm{odd }i, \textrm{even }j}$.
The two distributions are identical.

\bigskip

Finally, by \Cref{fact_tvd_chain_rule}, in the whole process, the players generated $\pis{\rv M_A}, \pis{\rv M_B}$ and $\rv\Pi_1$ such that the total variation distance to $\rv M_A$, $\rv M_B$ and $\rv\Pi_1$ following $\dist_{\pi\mid\Pyes}$ is at most
\[
	\frac{1}{2}\sqrt{k_{c,r-1}\cdot \Phi(m,c,C)}.
\]
This finalizes the proof of~\Cref{lem_th_dist_pstar}.

==> Files/setup.tex <==
% !TeX root = ../main.tex 
%!TEX root = ../main.tex


\section{The Basic Setup and Formalization of~\Cref{res:main}}\label{sec:OMC} 

We formalize~\Cref{res:main} in this section and present the basic setup for its proof. % and present the necessary definitions and a roadmap for its proof. 

\begin{theorem}
\label{thm:mainformal}
There is an absolute constant $\eta > 0$ such that the following holds: For even $k > 0$ and $n,r > 0$ such that $n$ is an odd multiple of $k$, any $r$-round communication protocol  $\pi$ that solves $\OMC_{n,k}$ with probability at least $(1/2+1/m^2)$ has communication cost $\norm{\pi} = 2^{-O(r)} \cdot (n/k)^{1-\eta\cdot k^{-1/(r-1)}}$.
\end{theorem}

\Cref{thm:mainformal} formalizes~\Cref{res:main}. Note that as for the notational convenience, we require the last message of the protocol to be the output, an $r$-round protocol for us corresponds to a ``standard $(r-1)$-round'' protocol, 
hence the term $r-1$ in~\Cref{thm:mainformal}. 

For the purpose of our lower bound, it would be easier to work with a more ``structured'' problem, called the \finalmatching (\FMT) problem, which we will define shortly. In the following, we start by introducing the basic definitions and then present the new problem and our main theorem on its communication complexity and a roadmap toward proving it. We conclude this section by showing that how~\Cref{thm:mainformal} can be derived from the lower bound for \FMT. The next two sections are then dedicated to completing the proof of the lower bound for  $\FMT$. 

\subsection{Layered Graphs}\label{sec:layered}
We start by defining a layered graph.

\begin{definition}
\label{def:layered}
Let $k > 0$ and $S = \{s_i\}_{i = 0}^k$ be a sequence of positive integers. An $S$-layered graph $G = (V, E)$ is such that $\card{V} = \sum_{i = 0}^k s_i$ and the following holds:

If $V = V_0 \sqcup V_1 \sqcup \cdots \sqcup V_k$ denotes the lexicographically smallest partition of $V$ into sets of size $s_0, s_1, \cdots, s_k$ respectively, then the set $E$ can be partitioned as $E = E_1 \sqcup \cdots \sqcup E_k$ such that for all $i \in [k]$, $E_i$ is a matching of size $\min(s_{i-1}, s_i)$ between $V_{i-1}$ and $V_i$.
\end{definition}

For a layered graph $G$, we call $V_0, V_1, \cdots, V_k$ the `layers' of $G$. In particular, $V_0$ is called the first layer and $V_k$ is called the last layer. When we wish to emphasize the partition $V = \bigsqcup_{i=0}^k V_i$, we write $G = \left(  \bigsqcup_{i=0}^k V_i, E\right)$. Similarly, we may write $G = \left(  \bigsqcup_{i=0}^k V_i, \bigsqcup_{i=1}^k E_i\right)$ if we also wish to emphasize the partition $E =\bigsqcup_{i=1}^k E_i$. 

As the edges in a layered graph $G$ form a matching between adjacent layers, any vertex in any layer of $G$ is connected to at most one other vertex in any other layer of $G$. We now make this formal. Let $i, i' \in \{0\} \cup [k]$ be given. Define the function $G^{\star}_{i' \to i} : V_{i'} \to V_i$ that takes a vertex $v \in V_{i'}$ as input, and outputs the unique vertex it is connected to in layer $V_i$, if there is one, and otherwise, outputs $\bot$. When $i' = i-1$, we abbreviate $G^{\star}_{i-1 \to i}$ as $G^{\star}_i$. We also abbreviate $G^{\star}_{0 \to k}$ as $G^{\star}$.


A layered graph is said to nice if for all $i, i' \in \{0\} \cup [k]$, the number of vertices $v$ in $V_{i'}$  such that $G^{\star}_{i' \to i}(v) = \bot$ is the smallest possible. Formally,
\begin{definition}
\label{def:nice}
Let $k > 0$ and $S = \{s_i\}_{i = 0}^k$ be a sequence of positive integers. An $S$-layered graph $G = (V, E)$ is said to be nice if, for all $i < i' \in \{0\} \cup [k]$, we have
\[
\card{\{ v \in V_{i'} \mid G^{\star}_{i' \to i}(v) \neq \bot\}} = \min_{i' \leq i'' \leq i} s_{i''}.
\]
\end{definition}




\subsection{Nested Block Graphs} \label{sec:nbg}

A particular type of layered graph needed to define the $\FMT$ problem is described in this section. We first fix some notation. For a non-empty sequence $S$, the notation $S[:-1]$ denotes the sequence $S$ without its last element. We use $\Vert$ to denote concatenation of two sequences. For some $s$ and $c > 0$, we use $s^{(c)}$ to denote the $c$-length sequence each of whose elements is $s$. 

Let $k > 0$ and $S = \{s_i\}_{i = 0}^k$ be a sequence of positive integers and $s, c > 0$. Define the sequence:
\begin{equation}
\label{eq:plug}
\plug_S(s,c) = s_0 \Vert s^{(c)} \Vert s_1 \Vert s^{(c)} \Vert s_2 \Vert \cdots \Vert s^{(c)} \Vert s_k.
\end{equation}
Namely, $\plug_S(s,c)$ plugs in $c$ occurrences of $s$ between any two elements in the sequence $S$. As a concrete example, we have $\plug_{1,3,5}(4,2) = 1,4,4,3,4,4,5$.

\begin{definition}
\label{def:nestseq}
Let $k > 0$ and $S = \{s_i\}_{i = 1}^k$ be an increasing sequence of positive integers. Let $c > 0$ be even. Define the sequence:
\[
\nest(S,c) = \begin{cases}
s_1^{(c + 1)} &, k = 1 \\
\plug_{\nest(S[:-1],c) \Vert s_1 }(s_{\card{S}},c - 1) &, k > 1
\end{cases}.
\]
Also, define $\n_{S,c}$ to be one less than the length of the sequence $\nest(S,c)$. We omit the subscripts when they are clear from context.
\end{definition}

We defer the intuition behind \Cref{def:nestseq} to the next subsection, but make here the following observations. 


\begin{observation}\label{obs:nest}
Let $k > 0$, $S = \{s_i\}_{i = 1}^k$ be an increasing sequence of positive integers, and $c > 0$ be even. It holds that:
\begin{enumerate}
\item \label{item:obs:nest1} $\n_{S,c} + 1 = \frac{ c^{\card{S} + 1} - 1 }{c-1} $ and is therefore, odd. 
\item \label{item:obs:nest2} The first and the last elements of $\nest(S,c)$ are both $s_1$.  So is the element at location $\n_{S,c} + 1  - c$.
\end{enumerate}
\end{observation}
We are now ready to define the notion of a nested block graph.

\begin{definition}[Nested block graphs]
\label{def:nbg}
Let $S = \{s_i\}_{i > 0}$ be an increasing sequence of positive integers and $c > 0$ be even. An $(S,c)$-nested block graph is an $\nest(S,c)$-layered graph that is nice.
\end{definition}

Often when we talk about nested block graphs, we will have a fixed set of vertices $V_{S,c} = \bigsqcup_{i=0}^{\n_{S,c}}V_{S,c,i}$ in mind and only consider different sets of edges on this fixed set of vertices. In particular, when we talk about a random $(S,c)$-nested block graph, we mean a graph chosen uniformly at random amongst all $(S,c)$-nested block graph on the vertex set $V_{S,c}$. For notational convenience, we use $\dist_{S,c}$ to denote the distribution that samples a random $(S,c)$-nested block graph and omit the subscripts from $\dist_{S, c}$ and $V_{S,c}$ when they are clear from context.




\subsection{The (Distributional) \finalmatching Problem}\label{sec:FMT}


For brevity, we define a \emph{distributional} version of the $\FMT$  problem directly. Recall our notation that if $G$ is a layered graph, then $G^{\star}$ is the function that takes a vertex in the first layer of $G$ to the unique vertex that it is connected to in the last layer $G$, if one exists, and to $\bot$ otherwise. Also, observe that \Cref{def:nice} ensures that $G^{\star}$ is never $\bot$ for any nested block graph $G$. In other words, for a nested block graph $G$, the function $G^{\star}$ is actually a bijection between the first and the last layer of $G$.


\begin{problem}[\bf{(Distributional) \finalmatching}] \label{prob:FMT}
Let $S = \{s_i\}_{i > 0}$ be an increasing sequence of positive integers and $c > 0$ be even. The $\FMT$ problem is a two player communication problem parametrized by $S$, $c$, and two bijections $\Y, \N: V_{0} \to V_{\n}$. Let $\dist^{\Y}$ (respectively, $\dist^{\N}$) denote the distribution $\dist$ conditioned on the event $G^{\star} = \Y$ (resp. $G^{\star} = \N$).

In the $(S,c,\Y,\N)$-\FMT problem, a graph $G = \left( \bigsqcup_{i=0}^{\n} V_{i}, \bigsqcup_{i=1}^{\n} E_{i} \right) $ is sampled uniformly at random from the distribution $\frac{1}{2} \cdot \dist^{\Y} + \frac{1}{2} \cdot \dist^{\N}$. Alice gets the edges $E_{i}$ for even $i$ and Bob gets the edges $E_{i}$ for odd $i$.  Both the players know the partition $V = \bigsqcup_{i=0}^{\n} V_{i}$. The task is output whether the function $G^{\star}$ equals $\Y$ or $\N$.



\end{problem}


Our main technical result is the following lower bound for the \FMT problem.~\Cref{thm:mainformal} then follows easily from this theorem as we show in~\Cref{sec:OMC}.  
\begin{theorem}
\label{thm:FMT}
There exists an absolute constant $\gamma$ such that the following holds: Let $r,m,c > 0$ be such that $m$ is a sufficiently large odd number and $c$ is a sufficiently large even number. Define the $r$-length sequence $S = m, m + \left\lfloor{\frac{m}{r-1}}\right\rfloor, m + \left\lfloor{\frac{2m}{r-1}}\right\rfloor, \cdots, 2m$.

For all distinct bijections $\Y, \N: V_0 \to V_{\n}$ and any $r$-round protocol $\prot$ for the $(S,c, \Y, \N)$-\FMT problem with probability of success at least $\frac{1}{2} + \frac{1}{m^2}$, we have that $\norm{\prot} \geq 2^{-\mathcal{O}(r)} \cdot m^{1 - \frac{1}{\gamma c}}$.
\end{theorem}

The proof of~\Cref{thm:FMT} consists of two main parts: 
\begin{inparaenum}[(I)]
\item \label{item:thm:FMT1} bounding the information revealed by the \emph{first message} of the protocol, and 
\item \label{item:thm:FMT2} a \emph{round elimination} argument that allows for ``shaving off'' the first message of the protocol without increasing its error by much on {a distribution} of smaller inputs. 
\end{inparaenum}
These parts can then be put together via an inductive argument that allows for removing 
every round of the protocol one by one and reduce the problem to a trivial protocol on a non-trivial distribution of inputs and finalize the proof. 


In the following, we formalize each part of the proof of~\Cref{thm:FMT} and show that how they can be put together to prove~\Cref{thm:FMT}. The next two sections of the paper are then dedicated to the proof of each of these parts separately. In both these parts, we exploit the fact that there is a simple recursive structure in the \FMT problem. This structure is best understood in light of \Cref{def:nestseq}. In  \Cref{def:nestseq}, the sequence $\nest(S,c)$ is obtained from the sequence $ \nest(S[:-1],c)$ as follows:
\begin{inparaenum}[(a)]
\item \label{item:structa} The element $s_1$ is appended to the sequence $\nest(S[:-1],c)$.
\item \label{item:structb} We plug in the element $s_{\card{S}}$ a total of $c-1$ times between any two elements of the appended sequence.
\end{inparaenum}



\paragraph{(\ref{item:thm:FMT1}) Information revealed by the first message.}  For this part of the proof, we restrict attention to \Cref{item:structb} above. Observe that \Cref{item:structb} ensures that the sequence $\nest(S,c)$ looks like a sequence of `blocks' of the form $s', s_{\card{S}}, s_{\card{S}}, \cdots, s_{\card{S}}, s''$ where the last layer of any block is merged with the first layer of the next block. We formalize this notion of block in the definition below:
\begin{definition}
\label{def:block}
Let $s, s', s'', c$ be integers such that $c$ is even and $\max(s', s'') < s$. An $(s, s', s'', c)$-block graph $G$ is a nice $S$-layered graph, where $S$ is the sequence $s' \Vert s^{(c-1)} \Vert s''$.
\end{definition}

Often when we talk about block graphs, we will have a fixed set of vertices $V_{s, s', s'', c} = \bigsqcup_{i = 0}^{c} V_{s, s', s'', c, i}$ in mind and only consider different edges on the vertices $V_{s, s', s'', c}$. In particular, when we say a random $(s, s', s'', c)$-block graph, we mean a graph chosen uniformly at random amongst all $(s, s', s'', c)$-block graphs on the vertex set $V_{s,s',s'',c}$. For notational convenience, we use $\dist^{\b}_{s, s', s'', c}$ to denote the distribution that samples a random $(s, s', s'', c)$-block graph and omit the subscripts when they are clear from context.

In the first part of the proof, we show that using one message, the parties cannot convey a lot of information about the function $G^{\star}$, for a random block graph $G$.

\newcommand{\lemoneroundjointunifcont}{
There exists an absolute constant $\gamma \in (0,1)$ such that the following holds: Let $s, s', s'', c$ be integers such that $c$ is a sufficiently large even number and $\max(s', s'') < s$. Suppose that $G = \left(  \bigsqcup_{i=0}^{c} V_i, \bigsqcup_{i=1}^c E_i\right)$ is a random $(s, s', s'', c)$-block graph drawn from the distribution $\dist^{\b}$, and Alice is given the edges $E_A = \{E_i\}_{\text{even } i}$ and Bob is given the edges $E_B = \{E_i\}_{\text{odd } i}$. Both players know the partition $\bigsqcup_{i=0}^{c} V_i$.

For all $C > 0$ and all one-way protocols $\prot$ of length $C$, {\em i.e.}, where Alice sends a single message $\Prot$ of length $C$ to Bob, we have 
\[
\mi{\rv{G^{\star}}}{\rv{\Prot}}[\rv{E}_B] \leq \Phi(s,\max(s',s''),c,C),
\]
 where:
\[
 \Phi(s,t,c,C) := s^2 \cdot \paren{ \frac{C}{\gamma \cdot \paren{s -t } } }^{c\gamma}
\]

}
\begin{lemma}[\textbf{Block Matchings After the First Round}]\label{lem_one_round_joint_unif}
	\lemoneroundjointunifcont
\end{lemma}

	
\paragraph{(\ref{item:thm:FMT2})  The round elimination argument.} The next part of the argument is to show that, for a sequence $S$ and $c > 0$, if a protocol for the $(S,c)$-\FMT problem\footnote{Technically, the \FMT problem is also parametrized by functions $\Y$ and $\N$ but we ignore these parameters in this informal overview.} does not reveal a lot of information about any of its block matchings (recall that \Cref{item:structb} ensures that the sequence $\nest(S,c)$ is a sequence of consecutive blocks) after the first round, we can use it to design a protocol for the $(S[:-1],c)$-\FMT problem with one fewer round.

To formalize this, we define $\rv{O}^{\prot}(G)$ to be the random variable that denotes the output of a protocol $\prot$ on input $G$. We have the following definition:

\begin{definition}
\label{def:adv}
Let $S = \{s_i\}_{i > 0}$ be an increasing sequence of positive integers and $c > 0$ be even. Let $\Y \neq \N$ be two distinct bijections $\Y, \N: V_{0} \to V_{\n}$ and let $\dist^{\Y}$ (respectively, $\dist^{\N}$) denote the distribution $\dist$ conditioned on the event $G^{\star} = \Y$ (resp. $G^{\star} = \N$). For $C > 0$ define:
\[
\adv(C,S,c,\Y,\N) := \sup \tvd{\distributions{\rv{O}^{\prot}(G)}{G \sim \dist^{\Y}}}{\distributions{\rv{O}^{\prot}(G)}{G \sim \dist^{\N}}}.
\]
where the supremum is taken over all $\card{S}$-round (possibly randomized) protocols $\prot$ for the $(S,c,\Y,\N)$-\FMT problem satisfying $\norm{\prot} \leq C$.
\end{definition}

That is, $\adv(C,S,c,\Y,\N)$ is how well a $C$-bit $\card{S}$-round protocol can distinguish between $\dist^{\Y}$ and $\dist^{\N}$, in terms of the total variation distance of the output.

\newcommand{\lemroundeliminationcont}{
Consider an increasing sequence $S = \{s_i\}_{i > 0}$ of sufficiently large numbers and a sufficiently large even number $c$. If $S$ has at least two elements and $S' = S[:-1]$, we have for all $C > 0$ that:
\begin{align*}
\max_{ \substack{\Y, \N : V_{S,c,0} \to V_{S,c,\n_{S,c}} \\ \Y \neq\N \text{ are bijections}} } \adv(C,S,c,\Y,\N) &\leq \max_{ \substack{\Y, \N : V_{S',c,0} \to V_{S',c,\n_{S',c}} \\ \Y \neq\N \text{ are bijections}} } \adv(C,S',c,\Y,\N) \\
&\hspace{3cm}  + \sqrt{\n_{S',c} \cdot  \Phi(s_{\card{S}},s_{\card{S'}},c,C)},
\end{align*}
where $\Phi(\cdot)$ is as defined in \Cref{lem_one_round_joint_unif}.
}
\begin{lemma}[\textbf{Round-Elimination}]\label{lem:round-elimination}
	\lemroundeliminationcont
\end{lemma}

\medskip

We now use \Cref{lem:round-elimination} to prove~\Cref{thm:FMT}. 




\begin{proof}[Proof of~\Cref{thm:FMT} (assuming~\Cref{lem:round-elimination})] 
For $i \in [r]$, denote by $S[:i]$ the $i$-length prefix of $S$ and let $C = \norm{\prot}$. Applying \Cref{lem:round-elimination} a total of $r-1$ times, once each for $S[:2], S[:3], \cdots, S$, we obtain:
\[
\adv(C,S,c,\Y,\N) \leq \max_{ \substack{\Y, \N : V_{S[:1],c,0} \to V_{S[:1],c,\n_{S[:1],c}} \\ \Y \neq\N \text{ are bijections}} } \adv(C,S[:1],c,\Y,\N)  + \sum_{i = 2}^{r} \sqrt{\n_{S[:i-1],c} \cdot  \Phi(s_{i},s_{i - 1},c,C)}.
\]
We claim that, for any distinct bijections $\Y, \N : V_{S[:1],c,0} \to V_{S[:1],c,\n_{S[:1],c}}$, we have that $\adv(C,S[:1],c,\Y,\N) = 0$. Indeed, by \Cref{def:adv}, we have that $\adv(C,S[:1],c,\Y,\N)$ is the total variation distance between the outputs generated by a $1$ round protocol when the graph $G$ is drawn from $\dist^{\Y}$ and when it is drawn from $\dist^{\N}$. In both cases, the marginal distribution of Alice's input and therefore, the marginal distribution of the output of the protocol (which is a function of Alice's input for a $1$-round protocol), is identical. As the distribution of the output is identical in the two cases, we have $\adv(C,S[:1],c,\Y,\N) = 0$. Plugging in, we get:
\[
\adv(C,S,c,\Y,\N) \leq \sum_{i = 2}^{r} \sqrt{\n_{S[:i-1],c} \cdot  \Phi(s_{i},s_{i - 1},c,C)}.
\]
We continue using \Cref{item:obs:nest1} of \Cref{obs:nest}. We have: 
\begin{equation}
\label{eq:FMT1}
\adv(C,S,c,\Y,\N) \leq \sum_{i = 2}^{r} \sqrt{ c^r \cdot  \Phi(s_{i},s_{i - 1},c,C)}.
\end{equation}
As $\prot$ is an $r$-round protocol for the $(S,c, \Y, \N)$-\FMT problem with probability of success at least $\frac{1}{2} + \frac{1}{m^2}$, we have:
\begin{align*}
\frac{1}{2} + \frac{1}{m^2} &\leq  \frac{1}{2} \cdot \Pr_{G \sim \dist^{\Y}}\paren{\rv{O}^{\prot}(G) = \Y} +\frac{1}{2} \cdot \Pr_{G \sim \dist^{\N}}\paren{\rv{O}^{\prot}(G) = \N} \\ 
&\leq \frac{1}{2} +   \frac{1}{2} \cdot \paren{ \Pr_{G \sim \dist^{\Y}}\paren{\rv{O}^{\prot}(G) = \Y} -  \Pr_{G \sim \dist^{\N}}\paren{\rv{O}^{\prot}(G) = \Y} } \\ 
&\leq \frac{1}{2} +   \adv(C,S,c,\Y,\N) .\tag{\Cref{def:adv}}
\end{align*}
Plugging into \eqref{eq:FMT1}, we have:
\[
\frac{1}{m^2} \leq \sum_{i = 2}^{r} \sqrt{ c^r \cdot  \Phi(s_{i},s_{i - 1},c,C)}.
\] 
Plugging in the definition of $\Phi(\cdot)$, we have: 
\[
\frac{1}{m^2} \leq \sum_{i = 2}^{r} \sqrt{ c^r \cdot  s_i^2 \cdot \paren{ \frac{C}{\gamma \cdot \paren{s_i - s_{i-1} } } }^{c\gamma}}.
\]
Using the definition of $S$ from \Cref{thm:FMT}, we get:
\[
\frac{1}{m^2} \leq \sum_{i = 2}^{r} \sqrt{ c^r \cdot  4m^2 \cdot \paren{ \frac{2Cr}{m \gamma } }^{c\gamma}} \leq r \cdot \sqrt{ c^r \cdot  4m^2 \cdot \paren{ \frac{2Cr}{m \gamma } }^{c\gamma}}.
\]
Rearranging gives:
\[
C \geq \frac{m \gamma}{2r} \cdot \paren{\frac{1}{4r^2} \cdot  \frac{1}{m^6} \cdot \frac{1}{   c^r }  }^{\frac{1}{c\gamma}}  \geq 2^{-\mathcal{O}(r)} \cdot m^{1 - \frac{6}{\gamma c}}.  \tag{as $1/c^{1/c}\geq \Omega(1)$}
\]
Re-parameterizing $\gamma$ by a constant factor proves the theorem.
\end{proof}

\subsection{The Lower Bound for $\cycle$ (\OMC)}\label{sec:OMC}

We now prove \Cref{thm:mainformal} based on~\Cref{thm:FMT}. 

\begin{proof}[Proof of~\Cref{thm:mainformal}]
% Proof by contradiction. Let $\delta = \gamma/100$ where $\gamma$ is the constant from \Cref{thm:FMT}. Suppose for the sake of contradiction that there exists $n,k,r > 0$ such that and an $r$-round protocol $\pi$ that solves $\OMC_{n,k}$ with probability $\geq \frac{2}{3}$ and satisfies $\norm{\pi} = o \Paren{ \frac{1}{k} \cdot \left(\frac{n}{k}\right) ^{1-   \frac{1}{\delta} \cdot  k^{-1/r} }}    $. 
Let us first assume that $k$ is a multiple of $4$, and let us fix an $r$-round protocol $\pi$ for $\OMC_{n,k}$ with probability of success at least $1/2+(k/n)^2$.
Let $m = n/k$ be an \emph{odd} integer (recall that $n$ is an odd multiple of $k$) and $c$ be the largest such that $k_{c,r}<k/4$. 
% {\color{red} Here, $k_0$ is the actual number of layers in our construction. Thus, $k_0 - 1$ is the number of matchings. Need replace $(3c)^r$ by the correct expression and make sure the last line is true}
Let $\Pyes$ be the matching such that $\Pyes(i) = (i + 1) \bmod m$ for all $i \in [m]$ and $\Pno$ be the identity matching on $m$ vertices, i.e., $\Pno(i) = i$ for all $i \in [m]$. 

We use $\pi$ to construct a protocol $\pi_{\fmt}$ for the $(m,c,r,\Pyes,\Pno)$-$\FMT$ problem on the distribution $\distFMT$.
Given as input an $(m,c,r)$-layered graph $G_{\fmt}$ (with $k_{c,r}+1$ layers) with Alice having the matchings for the even indexed layers and Bob having the matchings for the odd indexed layers, the protocol $\prot_{\fmt}$ behaves as follows: 
\begin{enumerate}[label=$(\arabic*)$]
\item Alice and Bob add $k/4 - (k_{c,r}+1)  $ new layers of vertices. For all $k_{c,r} \leq k' < k$, if $k'$ is odd, then Alice adds the identity matching between layer $k' - 1$ and layer $k' $ to her set of edges. Otherwise, Bob adds the identity matching to his set of edges.
\item The players make a copy of the graph, denoted by $\tilde G_{\fmt}$, with layers $\tilde V_0, \tilde V_1,\ldots,\tilde V_{k/4-1}$.
\item Bob adds the following edge to his input (see Figure~\ref{fig_proof_main_informal}):
	\begin{enumerate}
		\item an identity matching (i.e., $i$-th vertex to $i$-th vertex) between the top $m$ vertices in $V_{k/4-1}$ and the top $m$ vertices $\tilde V_0$,
		\item an identity matching between the top $m$ vertices in $\tilde V_{k/4-1}$ and the bottom $m$ vertices in $V_{0}$,
		\item an identity matching between the bottom $m$ vertices in $V_{k/4-1}$ and the bottom $m$ vertices in $\tilde V_{k/4-1}$,
		\item an identity matching between the bottom $m$ vertices in $\tilde V_0$ and the top $m$ vertices in $V_0$.
	\end{enumerate}
% \item Alice adds the identity matching between the layer $0$ and layer $k-1$ in $G_{\fmt}$ to her set of edges. Let $G_{\omc}$ be the new graph with the additional edges.
\item Alice and Bob run the protocol $\pi$ on the new graph $G_{\omc}$. 
% \item Output whatever $\Pi$ outputs.
\end{enumerate}
\begin{figure}
	\centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \begin{tikzpicture}
        	\draw[rectangle, rounded corners=2pt] (0, 0) rectangle (15pt, 40pt);
        	\draw[rectangle, rounded corners=2pt] (0, 45pt) rectangle (15pt, 85pt);
        	\draw[rectangle, rounded corners=2pt] (0, 100pt) rectangle (15pt, 140pt);
        	\draw[rectangle, rounded corners=2pt] (0, 145pt) rectangle (15pt, 185pt);

        	\draw[rectangle, rounded corners=2pt] (80pt, 0) rectangle (95pt, 40pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 45pt) rectangle (95pt, 85pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 100pt) rectangle (95pt, 140pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 145pt) rectangle (95pt, 185pt);

        	\node at (-10pt, 142.5pt) {$V_0$};
        	\node at (-10pt, 42.5pt) {$\tilde V_0$};
        	\node at (115pt, 142.5pt) {$V_{k/4-1}$};
        	\node at (115pt, 42.5pt) {$\tilde V_{k/4-1}$};

        	\draw (20pt, 20pt) edge [thick] node [above] {\scriptsize $i\mapsto \sigma(i)$} (75pt, 20pt);
        	\draw (20pt, 65pt) edge [thick] node [above] {\scriptsize $i\mapsto i+1$} (75pt, 65pt);
        	\draw (20pt, 120pt) edge [thick] node [above] {\scriptsize $i\mapsto \sigma(i)$} (75pt, 120pt);
        	\draw (20pt, 165pt) edge [thick] node [above] {\scriptsize $i\mapsto i+1$} (75pt, 165pt);

        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 165pt) -- (140pt, 165pt) -- (140pt, 90pt) -- (-25pt, 90pt) -- (-25pt, 65pt) -- (-5pt, 65pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 65pt) -- (120pt, 65pt) -- (120pt, 95pt) -- (-25pt, 95pt) -- (-25pt, 120pt) -- (-5pt, 120pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 120pt) -- (160pt, 120pt) -- (160pt, 20pt) -- (100pt, 20pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (-5pt, 20pt) -- (-45pt, 20pt) -- (-45pt, 165pt) -- (-5pt, 165pt);
        \end{tikzpicture}
        \caption{\scriptsize Vertex $i$ in top of $V_0$ connects to vertex $i+2$ in top of $V_0$.}\label{fig_sub_fig_Pyes}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.4\textwidth}
		\centering
       \begin{tikzpicture}
        	\draw[rectangle, rounded corners=2pt] (0, 0) rectangle (15pt, 40pt);
        	\draw[rectangle, rounded corners=2pt] (0, 45pt) rectangle (15pt, 85pt);
        	\draw[rectangle, rounded corners=2pt] (0, 100pt) rectangle (15pt, 140pt);
        	\draw[rectangle, rounded corners=2pt] (0, 145pt) rectangle (15pt, 185pt);

        	\draw[rectangle, rounded corners=2pt] (80pt, 0) rectangle (95pt, 40pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 45pt) rectangle (95pt, 85pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 100pt) rectangle (95pt, 140pt);
        	\draw[rectangle, rounded corners=2pt] (80pt, 145pt) rectangle (95pt, 185pt);

        	\node at (-10pt, 142.5pt) {$V_0$};
        	\node at (-10pt, 42.5pt) {$\tilde V_0$};
        	\node at (115pt, 142.5pt) {$V_{k/4-1}$};
        	\node at (115pt, 42.5pt) {$\tilde V_{k/4-1}$};

        	\draw (20pt, 20pt) edge [thick] node [above] {\scriptsize $i\mapsto \sigma'(i)$} (75pt, 20pt);
        	\draw (20pt, 65pt) edge [thick] node [above] {\scriptsize $i\mapsto i$} (75pt, 65pt);
        	\draw (20pt, 120pt) edge [thick] node [above] {\scriptsize $i\mapsto \sigma'(i)$} (75pt, 120pt);
        	\draw (20pt, 165pt) edge [thick] node [above] {\scriptsize $i\mapsto i$} (75pt, 165pt);

        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 165pt) -- (140pt, 165pt) -- (140pt, 90pt) -- (-25pt, 90pt) -- (-25pt, 65pt) -- (-5pt, 65pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 65pt) -- (120pt, 65pt) -- (120pt, 95pt) -- (-25pt, 95pt) -- (-25pt, 120pt) -- (-5pt, 120pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (100pt, 120pt) -- (160pt, 120pt) -- (160pt, 20pt) -- (100pt, 20pt);
        	\draw [line width=1.5pt, rounded corners=2pt] (-5pt, 20pt) -- (-45pt, 20pt) -- (-45pt, 165pt) -- (-5pt, 165pt);
        \end{tikzpicture}
		\caption{\scriptsize Vertex $i$ in top of $V_0$ connects to vertex $i$ in top of $V_0$.}\label{fig_sub_fig_Pno}
     \end{subfigure}
	\caption{Figure~\ref{fig_sub_fig_Pyes} and~\ref{fig_sub_fig_Pno} show the new graph $G_{\omc}$ when the final matching of $G_{\fmt}$ is $\Pyes$ and $\Pno$ respectively.}\label{fig_proof_main_informal}
\end{figure}

Suppose the matching from bottom $m$ vertices of $V_0$ to bottom $m$ vertices of $V_{k/4-1}$ is $\sigma$.
Observe that if $G_{\fmt}$ has final matching $\Pyes$, then the $i$-th vertex in top of $V_0$ connects to $(i+1)$-th vertex in top of $V_{k/4-1}$, which connects to $(i+1)$-th vertex in top of $\tilde V_0$, and $(i+2)$-th vertex in top of $\tilde V_{k/4-1}$.
Then it connects to $(i+2)$-th vertex in the bottom of $V_0$, which connects to the $\sigma(i+2)$-th vertex in the bottom of $V_{k/4-1}$, and then the $\sigma(i+2)$-th vertex in the bottom of $\tilde V_{k/4-1}$.
It then connects to the $(i+2)$-th vertex in the bottom of $\tilde V_0$, and finally, to the $(i+2)$-th vertex in the top of $V_0$.
Therefore, since $m$ is odd, all vertices are connected, and $G_{\omc}$ is simply a Hamiltonian cycle.
On the other hand, if $G_{\fmt}$ has final matching $\Pno$, one may verify similarly that $G_{\omc}$ has $n/k$ vertex-disjoint $k$-cycles.
This means that $\prot_{\fmt}$ has probability of success $\geq 1/2+1/m^2$. 
On the other hand, $\norm{\pi_{\fmt}}=\norm{\pi}$, and by \Cref{thm:FMT}, 
\[
\norm{\pi_{\fmt}} \geq 2^{-O(r)}\cdot m^{1-\frac6{\gamma c}}.
\]
% However, $\norm{\prot_{\fmt}} = \norm{\pi} =o \Paren{ \frac{1}{k} \cdot \left(\frac{n}{k}\right) ^{1-   \frac{1}{\delta} \cdot  k^{-1/r} }}  =   o \Paren{c^{-r} \cdot m ^{1-   \frac{2}{\gamma c} }}  $, a contradiction to~\Cref{thm:FMT}. 
By the fact that $k_{c,r}\leq 2\cdot (3c)^{r-1}$ and $k\leq k_{c+1,r}$, we get $c+1\geq\frac{1}{3}(k/2)^{1/(r-1)}\geq \frac{1}{6}k^{1/(r-1)}$, and thus, 
\begin{align*}
	\norm{\pi}&\geq 2^{-O(r)}\cdot m^{1-\frac6{\gamma c}} \\
	&\geq 2^{-O(r)} \cdot m^{1-\frac{36}{\gamma \cdot (k^{1/(r-1)}-6)}}.
\end{align*}
By setting $\eta=72/\gamma$, when $k^{1/(r-1)}\geq 12$, we get $\norm{\pi}\geq 2^{-O(r)} \cdot m^{1-{\eta}{}\cdot k^{-1/(r-1)}}$, proving the statement.
On the other hand, when $k^{1/(r-1)}<12$, the bound $2^{-O(r)} \cdot m^{1-{\eta}\cdot k^{-1/(r-1)}}<1$, and the statement holds trivially.
This proves the theorem when $k$ is a multiple of $4$.

In general, we make the same reduction for $k'=4\lfloor k/4\rfloor$ and $m=n/k$.
Then we split each vertex in the top of $V_0$ into a chain of length $k\bmod 4$.
The new graph has $m\cdot k'+m\cdot (k\bmod 4)=mk=n$ vertices.
Moreover,  if the graph is a Hamiltonian cycle before the split, then it remains a Hamiltonian cycle; if the graph was a disjoint union of $k'$-cycles, then the split adds $k\bmod 4=k-k'$ to the length of each cycle. 
Hence, this proves the theorem for all $k$.
\end{proof}

\begin{remark}
\label{rem:mainformal}
Observe that implicit in our proof above is a distribution $\mathcal{D}_{\mathsf{OMC}}$ for the $\OMC_{n, k}$ problem that is ``hard'' for $r$-rounds protocols. It is notable that $\mathcal{D}_{\mathsf{OMC}}$ can even be taken to be the uniform distribution that with probability $\frac{1}{2}$, is the uniform distribution over all Hamiltonian cycles and with probability $\frac{1}{2}$, is the uniform distribution on all graphs with $(n/k)$ vertex-disjoint $k$-cycles provided  that before running the protocol $\pi$, Alice and Bob permute the identity of the vertices randomly (using public randomness).
\end{remark}
\begin{remark}
\label{rem:arb_mat}
	By plugging in different pairs of $\Pyes$ and $\Pno$, we can prove lower bounds for distinguishing between different configurations of cycles in a graph.
	For example, by setting $\Pyes$ to the matching such that \[
		\Pyes(i)=\begin{cases}
			i-3 & \textrm{if $4\mid i$} \\
			i+1 & \textrm{otherwise}
		\end{cases}
	\]
	and $\Pno(i)=i$, and assuming $m=n/k$ is a multiple of four, the same argument proves that distinguishing between union of $2k$-cycles and $k$-cycles is hard.
	% In general, for any two specific configurations of lengths of cycles $(a_1,\ldots,a_l)$ such that $\sum_i a_i=n$ and $k\mid a_i$ for all $i$, one can set $\Pyes$ and $\Pno$ accordingly and prove that the two cases are hard to distinguish.
\end{remark}


